Graph-Time Convolutional Neural Networks: Architecture and Theoretical Analysis

Devising and analyzing learning models for spatiotemporal network data is of importance for tasks including forecasting, anomaly detection, and multi-agent coordination, among others. Graph Convolutional Neural Networks (GCNNs) are an established approach to learn from time-invariant network data. The graph convolution operation offers a principled approach to aggregate multiresolution information. However, extending the convolution principled learning and respective analysis to the spatiotemporal domain is challenging because spatiotemporal data have more intrinsic dependencies. Hence, a higher flexibility to capture jointly the spatial and the temporal dependencies is required to learn meaningful higher-order representations. Here, we leverage product graphs to represent the spatiotemporal dependencies in the data and introduce Graph-Time Convolutional Neural Networks (GTCNNs) as a principled architecture to aid learning. The proposed approach can work with any type of product graph and we also introduce a parametric product graph to learn also the spatiotemporal coupling. The convolution principle further allows a similar mathematical tractability as for GCNNs. In particular, the stability result shows GTCNNs are stable to spatial perturbations but there is an implicit trade-off between discriminability and robustness; i.e., the more complex the model, the less stable. Extensive numerical results on benchmark datasets corroborate our findings and show the GTCNN compares favorably with state-of-the-art solutions. We anticipate the GTCNN to be a starting point for more sophisticated models that achieve good performance but are also fundamentally grounded.

==> Figures/GT_Filter/gtfilter.tex <==
% !TEX root = ../main.tex

\def \thisplotscale {1.77}
\def \unit {\thisplotscale cm}

\tikzstyle {Phi} = [rectangle, 
thin,
minimum width = 1.15*\unit, 
minimum height = \sumshift*\unit, 
anchor = west,
draw,
fill = cyan!20]

\tikzstyle {sum} = [circle, 
thin,
minimum width  = 0.3*\unit, 
minimum height = 0.3*\unit, 
anchor = center,
draw,
fill = cyan!20]


\def \deltax {1.6}
\def \deltay {1.2}
\def \deltagat {1.2}
\def \sumshift {0.4}

{\footnotesize\begin{tikzpicture}[x = 1*\unit, y = 1*\unit]
		
		% Begin by drawing an empty node for initializing the chain
		\node (first) [] {};    
		
		% Draw the chain of graph shifts
		\path (first) ++ (0.30*\deltax, 0) node (0) [Phi] {$\bbI$};
		\path (0)     ++ (1.00*\deltax, 0) node (1) [Phi] {$\bbS_\diamond$};
		\path (1)     ++ (1.00*\deltax, 0) node (2) [Phi] {$\bbS_\diamond$};
%		\path (2)     ++ (1.00*\deltax, 0) node (3) [Phi] {$\bbPhi(\bbB, \bbe)$};
		
		% End by drawing an empty node for finalizing the chain
		\path (2.east) ++ (1*\sumshift*\deltax, 0) node [anchor=west] (last) [] {};
		
		% Draw the chain of GAT blocks
		%\path (0.west) ++ (0,\deltagat, 0)  node (GAT 0) [Phi] {$\bbB_1$, $\bbe_1$};
		%\path (1.west) ++ (0,\deltagat, 0)  node (GAT 1) [Phi] {$\bbB_2$, $\bbe_2$};
		%\path (2.west) ++ (0,\deltagat, 0)  node (GAT 2) [Phi] {$\bbB_3$, $\bbe_3$};
		%\path (3.west) ++ (0,\deltagat, 0)  node (GAT 3) [Phi] {$\bbB_4$, $\bbe_4$};
		
		% Draw the chain of additions
		\path (0.east) ++ (\sumshift*\deltax, -\deltay) node (sum0) [sum] {$+$};
		\path (1.east) ++ (\sumshift*\deltax, -\deltay) node (sum1) [sum] {$+$};
		\path (2.east) ++ (\sumshift*\deltax, -\deltay) node (sum2) [sum] {$+$};
%		\path (3.east) ++ (0.7*\sumshift*\deltax, -\deltay) node (sum3) [sum] {$+$};
		
		% Draw the arrows connecting the shift blocks
		\path[-stealth] (first) edge [above, pos=0.45] node {$\bbx_\diamond$}                 (0);	
		\path[-stealth] (0)     edge [above right, pos=0.0] node {$\bbS_\diamond^0\bbx_\diamond$}   (1);	
		\path[-stealth] (1)     edge [above right, pos=0.0] node {$\bbS_\diamond^1\bbx_\diamond$} (2);	
%		\path[-stealth] (2)     edge [above right, pos=0.0] node {$\ \bbPhi^{2}\bbX_{l-1}$} (last);
		\path[-]        (2)     edge [above right, pos=0.0] node {$\bbS_\diamond^2\bbx_\diamond$} (last);				
		
		% Draw the arrows connecting the GAT blocks to the shift blocks
		%\path (GAT 0) edge [right, pos=0.30] node {$\ \bbPhi^{(1)} (\bbB_1, \bbe_1)$}   (0);	
		%\path (GAT 1) edge [right, pos=0.30] node {$\ \bbPhi^{(2)} (\bbB_2, \bbe_2)$}   (1);	
		%\path (GAT 2) edge [right, pos=0.30] node {$\ \bbPhi^{(3)} (\bbB_3, \bbe_3)$}   (2);	
		%\path (GAT 3) edge [right, pos=0.30] node {$\ \bbPhi^{(4)} (\bbB_4, \bbe_4)$}   (3);	
		
		
		% Draw the arrows connecting to the sum blocks
		\path[-stealth, draw] (sum0 |- 0) -- node [left, pos=0.6 ] {$h_0$} (sum0);	
		\path[-stealth, draw] (sum1 |- 1) -- node [left, pos=0.6 ] {$h_1$} (sum1);	
		\path[-stealth, draw] (sum2 |- 2) -- node [left, pos=0.6 ] {$h_2$} (sum2);	
%		\path[-stealth, draw] (sum3 |- 3) -- node [left, pos=0.6 ] {$\ \bbPhi^{3}\bbX_{l-1}\bbA_2$} (sum3);	
		
		% Draw the arrows connecting the sum blocks
		\path[-stealth, draw] (sum0) -- (sum1);	
		\path[-stealth, draw] (sum1) -- (sum2);	
%		\path[-stealth, draw] (sum2) -- (sum3);	
		
		% Draw the convolution output
		\path[-stealth] (sum2) edge [above right, pos=0.0] node 
		{$\bby_\diamond = \sum_{k=0}^K h_k \bbS_\diamond^k \bbx_\diamond$} ++ (0.8*\deltax, 0);
		
		% Draw pictures
		\path (0)     ++ (0,0.5*\deltax) node (p0) [] {\includegraphics[width=0.2\linewidth]{Figures/GT_Filter/shape1.pdf}};
		\path (1)     ++ (0,0.5*\deltax) node (p1) [] {\includegraphics[width=0.2\linewidth]{Figures/GT_Filter/shape2.pdf}};
		\path (2)     ++ (0,0.5*\deltax) node (p2) [] {\includegraphics[width=0.2\linewidth]{Figures/GT_Filter/shape3.pdf}};
\end{tikzpicture}}

==> Figures/Lipschitz.tex <==

\begin{tikzpicture}
	
	\begin{axis}
		
		\addplot3 [domain=0:10,
		domain y = 0:1,
		samples = 20,
		samples y = 20,
		only marks,
		orange]{10*(sin(y))^3*x^2};
		
	\end{axis}
	
\end{tikzpicture}

==> GTCNN paper/Figures/GTCNN_BD.tex <==
% !TEX root = ../main.tex

\def \thisplotscale {1.77}
\def \unit {\thisplotscale cm}

\tikzstyle {Phi} = [rectangle, 
thin,
minimum width = 1.15*\unit, 
minimum height = \sumshift*\unit, 
anchor = west,
draw,
fill = cyan!20]

\tikzstyle {sum} = [circle, 
thin,
minimum width  = 0.3*\unit, 
minimum height = 0.3*\unit, 
anchor = center,
draw,
fill = cyan!20]


\def \deltax {1.6}
\def \deltay {1.2}
\def \deltagat {1.2}
\def \sumshift {0.4}

{\footnotesize\begin{tikzpicture}[x = 1*\unit, y = 1*\unit]
		
		\pgfdeclarelayer{bg}    % declare background layer
		\pgfsetlayers{bg,main}  % set the order of the layers (main is the standard layer)
		
		
		% Begin by drawing an empty node for initializing the chain
		\node (first) [] {};    
		
		% layer1
		\path (first) ++ (0.30*\deltax, 0) node (0) [Phi] {$\bbH_1(\bbS_\diamond)$};
		\path (0)     ++ (0.75*\deltax, 0) node (1) [Phi] {$\sigma(\cdot)$};
		% layer2
		\path (first) ++ (0.30*\deltax, -0.6*\deltax) node (2) [Phi] {$\bbH_2(\bbS_\diamond)$};
		\path (2)     ++ (0.75*\deltax, 0) node (3) [Phi] {$\sigma(\cdot)$};
		% layer3
		\path (first) ++ (0.30*\deltax, -0.6*2*\deltax) node (4) [Phi] {$\bbH_3(\bbS_\diamond)$};
		\path (4)     ++ (0.75*\deltax, 0) node (5) [Phi] {$\sigma(\cdot)$};
		
		% End by drawing an empty node for finalizing the chain
		\path (5.east) ++ (1*\sumshift*\deltax, 0) node [anchor=west] (last) [] {};
		
		% defining connector nodes
		\path (1) ++ (0, -0.3*\deltax) coordinate [] (1c) [] {};
		\path (0) ++ (0, -0.3*\deltax) coordinate [] (2c) [] {};
		\path (3) ++ (0, -0.3*\deltax) coordinate [] (3c) [] {};
		\path (2) ++ (0, -0.3*\deltax) coordinate [] (4c) [] {};

		
		% Draw connectors in each layer
		\path[-stealth] (first) edge [above, pos=-0.5] node {$\bbx_{\diamond,0}=\bbx_\diamond$}                 (0);	
		\path[-stealth] (0)     edge [above right, pos=0.0] node {}   (1);	
		\path[-stealth] (2)     edge [above right, pos=0.0] node {}   (3);	
		\path[-stealth] (4)     edge [above right, pos=0.0] node {}   (5);		
		
		% Draw connectors between layers
		\path[] (1) edge [above, pos=0.45] node {} (1c);
		\path[-stealth] (2c) edge [above left, pos=0.45] node {$\bbx_{\diamond,1}$} (2);
		\path[] (2c) edge [above, pos=0.45] node {} (1c);
		
		\path[] (3) edge [above, pos=0.45] node {} (3c);
		\path[-stealth] (4c) edge [above left, pos=0.45] node {$\bbx_{\diamond,2}$} (4);
		\path[] (4c) edge [above, pos=0.45] node {} (3c);

		% Draw the convolution output
		\path[-stealth] (5) edge [above right, pos=0.1] node 
		{$\Phi(\bbx_\diamond;\ccalH(\bbS_\diamond))$} ++ (0.8*\deltax, 0);
		
		% Draw box around layers
		\begin{pgfonlayer}{bg}
			\node[fit=(0)(1), draw,inner sep = 4*\deltax,fill = red!30, fill opacity = 0.5,draw = white, rounded corners=10](l1) {};
			\node[fit=(2)(3), draw,inner sep = 4*\deltax,fill = red!30, fill opacity = 0.5,draw = white, rounded corners=10](l2) {};
			\node[fit=(4)(5), draw,inner sep = 4*\deltax,fill = red!30, fill opacity = 0.5,draw = white, rounded corners=10](l3) {};
		\end{pgfonlayer}

		% Write the layer names
		\node[below] at (l1.north) {\tiny Layer 1};
		\node[below] at (l2.north) {\tiny Layer 2};
		\node[below] at (l3.north) {\tiny Layer 3};
\end{tikzpicture}}

==> GTCNN paper/Figures/GT_Filter/gtfilter.tex <==
% !TEX root = ../main.tex

\def \thisplotscale {1.77}
\def \unit {\thisplotscale cm}

\tikzstyle {Phi} = [rectangle, 
thin,
minimum width = 1.15*\unit, 
minimum height = \sumshift*\unit, 
anchor = west,
draw,
fill = cyan!20]

\tikzstyle {sum} = [circle, 
thin,
minimum width  = 0.3*\unit, 
minimum height = 0.3*\unit, 
anchor = center,
draw,
fill = cyan!20]


\def \deltax {1.6}
\def \deltay {1.2}
\def \deltagat {1.2}
\def \sumshift {0.4}

{\footnotesize\begin{tikzpicture}[x = 1*\unit, y = 1*\unit]
		
		% Begin by drawing an empty node for initializing the chain
		\node (first) [] {};    
		
		% Draw the chain of graph shifts
		\path (first) ++ (0.30*\deltax, 0) node (0) [Phi] {$\bbI$};
		\path (0)     ++ (1.00*\deltax, 0) node (1) [Phi] {$\bbS_\diamond$};
		\path (1)     ++ (1.00*\deltax, 0) node (2) [Phi] {$\bbS_\diamond$};
%		\path (2)     ++ (1.00*\deltax, 0) node (3) [Phi] {$\bbPhi(\bbB, \bbe)$};
		
		% End by drawing an empty node for finalizing the chain
		\path (2.east) ++ (1*\sumshift*\deltax, 0) node [anchor=west] (last) [] {};
		
		% Draw the chain of GAT blocks
		%\path (0.west) ++ (0,\deltagat, 0)  node (GAT 0) [Phi] {$\bbB_1$, $\bbe_1$};
		%\path (1.west) ++ (0,\deltagat, 0)  node (GAT 1) [Phi] {$\bbB_2$, $\bbe_2$};
		%\path (2.west) ++ (0,\deltagat, 0)  node (GAT 2) [Phi] {$\bbB_3$, $\bbe_3$};
		%\path (3.west) ++ (0,\deltagat, 0)  node (GAT 3) [Phi] {$\bbB_4$, $\bbe_4$};
		
		% Draw the chain of additions
		\path (0.east) ++ (\sumshift*\deltax, -\deltay) node (sum0) [sum] {$+$};
		\path (1.east) ++ (\sumshift*\deltax, -\deltay) node (sum1) [sum] {$+$};
		\path (2.east) ++ (\sumshift*\deltax, -\deltay) node (sum2) [sum] {$+$};
%		\path (3.east) ++ (0.7*\sumshift*\deltax, -\deltay) node (sum3) [sum] {$+$};
		
		% Draw the arrows connecting the shift blocks
		\path[-stealth] (first) edge [above, pos=0.45] node {$\bbx_\diamond$}                 (0);	
		\path[-stealth] (0)     edge [above right, pos=0.0] node {$\bbS_\diamond^0\bbx_\diamond$}   (1);	
		\path[-stealth] (1)     edge [above right, pos=0.0] node {$\bbS_\diamond^1\bbx_\diamond$} (2);	
%		\path[-stealth] (2)     edge [above right, pos=0.0] node {$\ \bbPhi^{2}\bbX_{l-1}$} (last);
		\path[-]        (2)     edge [above right, pos=0.0] node {$\bbS_\diamond^2\bbx_\diamond$} (last);				
		
		% Draw the arrows connecting the GAT blocks to the shift blocks
		%\path (GAT 0) edge [right, pos=0.30] node {$\ \bbPhi^{(1)} (\bbB_1, \bbe_1)$}   (0);	
		%\path (GAT 1) edge [right, pos=0.30] node {$\ \bbPhi^{(2)} (\bbB_2, \bbe_2)$}   (1);	
		%\path (GAT 2) edge [right, pos=0.30] node {$\ \bbPhi^{(3)} (\bbB_3, \bbe_3)$}   (2);	
		%\path (GAT 3) edge [right, pos=0.30] node {$\ \bbPhi^{(4)} (\bbB_4, \bbe_4)$}   (3);	
		
		
		% Draw the arrows connecting to the sum blocks
		\path[-stealth, draw] (sum0 |- 0) -- node [left, pos=0.6 ] {$h_0$} (sum0);	
		\path[-stealth, draw] (sum1 |- 1) -- node [left, pos=0.6 ] {$h_1$} (sum1);	
		\path[-stealth, draw] (sum2 |- 2) -- node [left, pos=0.6 ] {$h_2$} (sum2);	
%		\path[-stealth, draw] (sum3 |- 3) -- node [left, pos=0.6 ] {$\ \bbPhi^{3}\bbX_{l-1}\bbA_2$} (sum3);	
		
		% Draw the arrows connecting the sum blocks
		\path[-stealth, draw] (sum0) -- (sum1);	
		\path[-stealth, draw] (sum1) -- (sum2);	
%		\path[-stealth, draw] (sum2) -- (sum3);	
		
		% Draw the convolution output
		\path[-stealth] (sum2) edge [above right, pos=0.0] node 
		{$\bby_\diamond = \sum_{k=0}^K h_k \bbS_\diamond^k \bbx_\diamond$} ++ (0.8*\deltax, 0);
		
		% Draw pictures
		\path (0)     ++ (0,0.5*\deltax) node (p0) [] {\includegraphics[width=0.2\linewidth]{Figures/GT_Filter/shape1.pdf}};
		\path (1)     ++ (0,0.5*\deltax) node (p1) [] {\includegraphics[width=0.2\linewidth]{Figures/GT_Filter/shape2.pdf}};
		\path (2)     ++ (0,0.5*\deltax) node (p2) [] {\includegraphics[width=0.2\linewidth]{Figures/GT_Filter/shape3.pdf}};
\end{tikzpicture}}

==> GTCNN paper/Figures/GT_Filter/gtfilter_kron.tex <==
% !TEX root = ../main.tex

\def \thisplotscale {2}
\def \unit {\thisplotscale cm}

\tikzstyle {Phi} = [rectangle, 
thin,
minimum width = 1.15*\unit, 
minimum height = \sumshift*\unit, 
anchor = west,
draw,
fill = cyan!20]

\tikzstyle {sum} = [circle, 
thin,
minimum width  = 0.3*\unit, 
minimum height = 0.3*\unit, 
anchor = center,
draw,
fill = cyan!20]


\def \deltax {1.6}
\def \deltay {1.2}
\def \deltagat {1.2}
\def \sumshift {0.4}

{\footnotesize\begin{tikzpicture}[x = 1*\unit, y = 1*\unit]
		
		\pgfdeclarelayer{bg}    % declare background layer
		\pgfsetlayers{bg,main}
		% Begin by drawing an empty node for initializing the chain
		\node (first) [] {};  
		
		% Draw the chain of graph shifts
		\path (first) ++ (0, -0.30*\deltay) node (0) [Phi] {$\bbI$};
		\path (0)     ++ (-1.15*\unit/2, -1.00*\deltay) node (1) [Phi] {$\bbS_\diamond$};
		\path (1)     ++ (-1.15*\unit/2, -1.00*\deltay) node (2) [Phi] {$\bbS_\diamond$};
		
		% End by drawing an empty node for finalizing the chain
		\path (2.south) ++ (0, -1.25*\sumshift*\deltay) node [anchor=south] (last) [] {};
		\path (0.north) ++ (0, 1*\sumshift*\deltay) node [anchor=north] (input) [] {};
		
		% Draw the chain of additions
		\path (0.south) ++ (\deltax, -\sumshift*\deltay) node (sum0) [sum] {$+$};
		\path (1.south) ++ (\deltax, -\sumshift*\deltay) node (sum1) [sum] {$+$};
		\path (2.south) ++ (\deltax, -\sumshift*\deltay) node (sum2) [sum] {$+$};
		
		% Draw the arrows connecting the shift blocks
		\path[-stealth] (input) edge [above, pos=0.0] node {$\bbx_\diamond$}                 (0);	
		\path[-stealth] (0)     edge [below left, pos=0.0] node {$\bbS_\diamond^0\bbx_\diamond$}   (1);	
		\path[-stealth] (1)     edge [below left, pos=0.0] node {$\bbS_\diamond^1\bbx_\diamond$} (2);	
		\path[-]        (2)     edge [below left, pos=0.0] node {$\bbS_\diamond^2\bbx_\diamond$} (last);				
		
		% Draw the arrows connecting to the sum blocks
		\path[-stealth, draw] (sum0 -| 0) -- node [above, pos=0.6 ] {$h_0$} (sum0);	
		\path[-stealth, draw] (sum1 -| 1) -- node [above, pos=0.6 ] {$h_1$} (sum1);	
		\path[-stealth, draw] (sum2 -| 2) -- node [above, pos=0.6 ] {$h_2$} (sum2);	
%	
		
		% Draw the arrows connecting the sum blocks
		\path[-stealth, draw] (sum0) -- (sum1);	
		\path[-stealth, draw] (sum1) -- (sum2);	

		
		% Draw the convolution output
		\path[-stealth] (sum2) edge [above right, pos= 0.5] node 
		{$\bby_\diamond$} ++ (0.25*\deltax, 0);
		
		% Draw pictures
		\path (0)     ++ (-1.1*\deltax,-0.15) node (p0) [] {\includegraphics[width=0.2\linewidth]{Figures/GT_Filter/kron0.pdf}}
		++ (-1.3*\deltax,0) node (p01) [] {\includegraphics[width=0.2\linewidth]{Figures/GT_Filter/cart0.pdf}}
		++ (-1.3*\deltax,0) node (p02) [] {\includegraphics[width=0.2\linewidth]{Figures/GT_Filter/strong0.pdf}};
		
		\path (1)     ++ (-1.1*\deltax,-0.15) node (p1) [] {\includegraphics[width=0.2\linewidth]{Figures/GT_Filter/kron1.pdf}}
		++ (-1.3*\deltax,0) node (p11) [] {\includegraphics[width=0.2\linewidth]{Figures/GT_Filter/cart1.pdf}}
		++ (-1.3*\deltax,0) node (p12) [] {\includegraphics[width=0.2\linewidth]{Figures/GT_Filter/strong1.pdf}};
		
		\path (2)     ++ (-1.1*\deltax,-0.15) node (p2) [] {\includegraphics[width=0.2\linewidth]{Figures/GT_Filter/kron2.pdf}}++ (-1.3*\deltax,0) node (p21) [] {\includegraphics[width=0.2\linewidth]{Figures/GT_Filter/cart2.pdf}}
		++ (-1.3*\deltax,0) node (p22) [] {\includegraphics[width=0.2\linewidth]{Figures/GT_Filter/strong2.pdf}};
		
		\path (input)
		++ (-1.1*\deltax,0.05) node (pg1) [] {Kronecker}
		++ (-1.3*\deltax,0) node (pg2) [] {Cartesian}
		++ (-1.3*\deltax,0) node (pg3) [] {Strong};
		
				% Draw box around layers
		\begin{pgfonlayer}{bg}
			\node[fit=(0)(1)(2)(sum0)(sum1)(sum2), draw,inner sep = 4*\deltax,fill = red!30, fill opacity = 0.5,draw = white, rounded corners=10](l1) {};
%			\node[fit=(2)(3), draw,inner sep = 4*\deltax,fill = red!30, fill opacity = 0.5,draw = white, rounded corners=10](l2) {};
%			\node[fit=(4)(5), draw,inner sep = 4*\deltax,fill = red!30, fill opacity = 0.5,draw = white, rounded corners=10](l3) {};
		\end{pgfonlayer}
		
\end{tikzpicture}}

==> GTCNN paper/Figures/Lipschitz.tex <==

\begin{tikzpicture}
	
	\begin{axis}
		
		\addplot3 [domain=0:10,
		domain y = 0:1,
		samples = 20,
		samples y = 20,
		only marks,
		orange]{10*(sin(y))^3*x^2};
		
	\end{axis}
	
\end{tikzpicture}

==> GTCNN paper/Figures/table2.tex <==

\begin{tabular}{|ll|lll|lll|lll|}
	\hline
	\multirow{2}{*}{Data}     & \multirow{2}{*}{Models} & \multicolumn{3}{c|}{1-Steps}                    & \multicolumn{3}{c|}{3-Steps}                    & \multicolumn{3}{c|}{5-Steps}                    \\ \cline{3-11} 
	&                         & MAE           & RMSE          & MAPE            & MAE           & RMSE          & MAPE            & MAE           & RMSE          & MAPE             \\ \hline
	\multirow{8}{*}{\begin{sideways}Moelene\end{sideways}}
	& ARIMA~\cite{li2017diffusion}                   
	& 2.26          & 4.74         & 5.24\%          & 3.56          & 7.95         & 12.37\%         & 6.15          & 13.59         & 17.51\%          \\
	& G-VARMA~\cite{mo:isufi2019VARMA}                 
	& \textbf{2.09}         & \textbf{4.40}          & \textbf{4.97\%}          & \textbf{3.45}          & \textbf{7.69}         & \textbf{12.07\% }        & \textbf{6.00 }         & \textbf{13.26 }         & \textbf{17.42\%}          \\
	& GP-VAR~\cite{mo:isufi2019VARMA}                  
	& \ul{2.13}         & \ul{4.47}          & \ul{5.01\% }         & \ul{3.52}          & \ul{7.85}          & \ul{12.10\%}         & \ul{6.05}          & \ul{13.38}          & \ul{17.46\% }         \\
	& LSTM
	& 3.84          & 8.06          & 12.44\%          & 4.72          & 10.52          & 15.54\%         & 7.84         & 17.33          & 21.09\%          \\
	& Graph Wavenet~\cite{mo:wu2019graph}           
	& 3.52     & 7.41 & 11.39\%     & 4.49     & 10.02     & 15.11\%     & 7.54 & 16.66     & 20.14\% \\
	& STGCN~\cite{mo:yu2017spatio}                   
	& 3.78          & 7.95          & 15.20\%          & 4.56          & 10.18          & 9.57\%          & 7.50          & 16.59         & 20.12\%          \\
	& GGRNN~\cite{mo:ruiz2020gatedGRNN}                  
	& 3.17         & 6.67          & 15.20\%          & 4.55          & 10.16          & 8.97\%          & 7.35          & 16.26          & 19.89\%          \\
	& GTCNN (this work)
	& 3.55 & 7.47     & 11.45\% & 4.43 & 9.87 & 14.98\% & 6.54     & 14.46 & 18.53\%          \\ \hline
	\multirow{8}{*}{\begin{sideways}NOAA\end{sideways}}
	& ARIMA~\cite{li2017diffusion}                  
	& 0.39          & 0.98         & 1.68\%          & 1.60          & 3.86         & 4.21\%          & 2.89         & 6.75          & 8.47\%           \\
	& G-VARMA~\cite{mo:isufi2019VARMA}                 
	& 0.36         & 0.89         & 1.67\%          & 1.39         & 3.35          & 3.56\%          & 2.59         & 5.48          & 6.92\%           \\
	& GP-VAR~\cite{mo:isufi2019VARMA}                  
	& 0.41       & 1.02         & 1.70\%          & 1.40          & 3.37          & 3.56\%          & 2.59          & 6.04          & 7.31\%           \\
	& LSTM                    & 0.29          & 0.75          & 1.58\%          & \ul{0.66 }         & \ul{1.59}          & \ul{2.31\%}          & \textbf{1.39 }         & \textbf{3.24 }         & \textbf{3.46\% }          \\
	& Graph Wavenet~\cite{mo:wu2019graph}           
	& 0.33     & 0.83     & 1.65\%    & 0.95 & 2.28     & 2.84\%  &\ul{ 1.42} & \ul{3.31} & \ul{3.51\% } \\
	& STGCN~\cite{mo:yu2017spatio}                   
	& 0.35          & 0.87          & 1.65\%          & 0.82          & 1.97          & 2.44\%          & 1.68         & 3.91          & 3.92\%           \\
	& GGRNN~\cite{mo:ruiz2020gatedGRNN}                   
	& \textbf{0.26}          & \textbf{0.64}          & \textbf{1.54\%}          & 0.84          & 2.02          & 2.47\%     & 1.63          & 3.80         & 3.89\%           \\
	& GTCNN (this work)                   &\ul{ 0.28 }& \ul{0.70} & \ul{1.57\%} &\textbf{ 0.63}     & \textbf{1.53 } & \textbf{2.28\% }         & 1.53     & 3.57     & 3.65\%      \\ \hline
\end{tabular}


==> GTCNN paper/Sections/Background.tex <==
Here, we first introduce some background material about product graphs and their use to represent multivariate time-series. Then, we motivate the problem of learning from multivariate time-series via an inductive bias perspective.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 						SECTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Product Graphs for Spatiotemporal Coupling}\label{subsec_PG}
%product graphs aim at representing a multivariate temporal recursion as a static graph signal over a larger graphs capturing both spatial and temporal relations \cite{hammack2011handbook}. Product graphs arise in several fields, including biology and  finance. They can  decompose large graphs, alleviating storage requirements and computational efforts.
%
%A scalar time series can be seen as a graph signal residing on top of a line graph, where each node of the graph represents the discrete time index. When we have a multivariate time series residing on top of a network, two graphs can be used to represent such setting: \textit{i)} the line graph for  each time series;  and \textit{ii)} the spatial graph, to capture dependencies among time series. Product graphs enable us to have a unified and combined picture of this spatio-temporal dataset, by combining the two graphs into a larger one.

Consider an $N \times 1$ multivariate signal $\bbx_t$ collected over $T$ time instances in matrix $\bbX = [\bbx_1, \ldots, \bbx_T ]$. The $t$th column $\bbx_t = [x_t(1), \ldots, x_t(N)]^\top$ may be measurements of different sensors in a sensor network at time $t$, whereas the $i$th row $\bbx^i = [x_1(i), \ldots, x_T(i)]^\top$ may be the time series of sensor $i$ over the $T$ time instants. When learning representations from the data in $\bbX$ we are interested in exploiting both the spatial dependencies in $\bbx_t$ and the temporal dependencies in $\bbx^i$. However, despite learning from these spatial and temporal relations is important to extract patterns in $\bbX$, we need to devise methods that exploit them \emph{jointly} as an inductive bias for learning representations~\cite{battaglia2018inductivebias}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FIGURE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.7\linewidth]{Figures/Fig1}
	\end{center}
	\caption{Spatial and temporal graphs along with signals over their nodes. (Left) Spatial graph and graph signal at time $t$. Scalar $x_t(2)$ is the signal and node two recorded at time $t$. It is proximal with signals at nodes one, three, and four. (Right) Temporal graph and $i$th time series illustrated as graph signal. Edges in green are those of a directed line graph, while edges green and grey are of a cyclic graph.}
	\label{fig: signal over graphs}	
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

When data $\bbx_t$ have a (hidden) underlying structure, we can capture their \textit{spatial} relations through a \textit{spatial graph} $\ccalG = (\ccalV, \ccalE)$ of $N$ nodes in set $\ccalV = \{1, \ldots , N\}$ and $|\ccalE|$ edges in set $\ccalE \subseteq \ccalV \times \ccalV$. We represent the structure of $\ccalG$ via its graph shift operator (GSO) matrix $\bbS \in  \reals^{N \times N}$ which is a sparse matrix with non-zero entries $[\bbS]_{ij} \neq 0$ only if $(i,j) \in \ccalE$ or $i = j$~\cite{ortega2018overview}. We can view $\bbx_t$ as a graph signal with scalar $x_t(i)$ residing on node $i$. Likewise, we can capture the \textit{temporal} relations in $\bbx^i$ through a \textit{temporal graph} $\ccalG_T = (\ccalV_T , \ccalE_T )$ of $T$ nodes in set $\ccalV_T = \{1, \ldots, T\}$
and $|\ccalE_T |$ edges in set $\ccalE_T \in \ccalV_T \times \ccalV_T$. Each node represents one time instant $t$ and set $\ccalE_T$ contains an edge if signals at instances $t$ and $t^\prime$ are related. Also, we represent the structure of $\ccalG_T$ with its GSO matrix $\bbS_T \in \reals^{T \times T}$. Data $\bbx^i$ can be seen as a graph signal with scalar $x_t(i)$ being the value at node $t$. Examples of $\ccalG_T$ are the directed line graph that assumes signal $x_t(i)$ depends only on the former instance $x_{t-1}(i)$, the cyclic graph that accounts for periodicity, or any other graph that encodes the temporal dependencies in $\bbx^i$, see Fig.~\ref{fig: signal over graphs}.

Given graphs $\ccalG$, $\ccalG_T$, we can capture the spatiotemporal relations in the data $\bbX$ through product graphs
%
\begin{equation}
\mathcal{G}_{\diamond}=   \mathcal{G}_{T}   \diamond \mathcal{G} =\left(\mathcal{V}_{\diamond}, \mathcal{E}_{\diamond} ,\mathbf{S}_{\diamond}\right).
\end{equation}
%
The node set $\ccalV_\diamond= \ccalV_T \times \ccalV$ is the Cartesian product between $\ccalV_T$ and $\ccalV$ with cardinality $|\mathcal{V}_{\diamond}|=NT$ and node $i_\diamond \in \ccalV$ represents the space-time location $(i,t)$; see Fig.~\ref{fig: product graph}. The edge set $\ccalE_\diamond \subseteq \mathcal{V}_\diamond \times \mathcal{V}_\diamond$ connects now space-time locations, which structure and respective GSO $\bbS_\diamond \in \reals ^{NT \times NT}$ are dictated by the type of product graph. Typical product graphs are~\cite{sandryhaila2014big}:
%%%%%%%%%%%%%%%%%
\begin{itemize}
	\item \textit{Kronecker product}: $\ccalG_{\otimes} = \ccalG_T {\otimes} \ccalG = (\ccalV_{\otimes}, \ccalE_\otimes, \bbS_\otimes)$ has the GSO $\bbS_{\otimes}=\bbS_T \otimes \bbS$. The number of edges is $|\ccalE_\otimes| = 2|\ccalE| |\ccalE_T|$. The Kronecker product translates the spatial coupling into a temporal coupling in which spatiotemporal nodes $i_\diamond = (i,t)$ and $j_\diamond = (j,t+1)$ are connected only if the spatial nodes $i,j$ are connected in $\ccalG$ and the temporal nodes $t$ and $t+1$ are connected in $\ccalG_T$; grey edges in Fig.~\ref{fig: product graph}.
	%
	\medskip
	%
	\item \textit{Cartesian product}: $\ccalG_{\times} = \ccalG_T {\times} \ccalG = (\ccalV_{\times}, \ccalE_\times, \bbS_\times)$ has the GSO $\mathbf{S}_{ \times}=\mathbf{S}_T \otimes \mathbf{I}_{N}+\mathbf{I}_{T} \otimes \mathbf{S}$. The number of edges is $|\ccalE_\times| = T|\ccalE| + N|\ccalE_T|$. The Cartesian product implies a temporal coupling by connecting each spatial node to itself in consecutive instants as dictated by $\ccalG_T$, i.e., the spatiotemporal nodes $i_\diamond = (i,t)$ and $j_\diamond = (i,t+1)$ are connected if time instants $t$ and $t+1$ are adjacent; red and green edges in Fig.~\ref{fig: product graph}.
	
	%
	\medskip
	%
	\item \textit{Strong product}: $\ccalG_{\boxtimes} = \ccalG_T {\boxtimes} \ccalG = (\ccalV_{\boxtimes}, \ccalE_\boxtimes, \bbS_\boxtimes)$ has the GSO $\bbS_{\boxtimes}=\mathbf{S}_T \otimes \mathbf{I}_{N}+\mathbf{I}_{T} \otimes \mathbf{S} + \bbS_T \otimes \bbS$. The number of edges is $|\ccalE_\boxtimes| = |\ccalE| |\ccalE_T| + T|\ccalE| + N|\ccalE_T|$. The strong product is the union of the Kronecker and Cartesian products. Here, spatiotemporal nodes $i_\diamond = (i,t)$ and $j_\diamond=(j,t+1)$ are connected if time instants $t$ and $t+1$ are adjacent in the temporal graph $\ccalG_T$ and spatial nodes $i$ and $j$ are either neighbors or $i=j$ in graph $\ccalG$; red, green, and grey edges in Fig.~\ref{fig: product graph}.
	
\end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
	\begin{center}
		\includegraphics[width=\linewidth]{Figures/Fig2}
	\end{center}
	\caption{Different product graphs and the formation of multivariate temporal data over them. (grey edges) Kronecker product $\ccalG_{\otimes} = \ccalG_T {\otimes} \ccalG$. (green and red edges) Cartesian product $\ccalG_{\times} = \ccalG_T {\times} \ccalG$. (All edges) Strong product $\ccalG_{\boxtimes} = \ccalG_T {\boxtimes} \ccalG.$}
	\label{fig: product graph}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%

%All the aforementioned product graphs can be generalized through a parametric model, called parametric product graph \cite{natali2020forecasting}, which has the GSO
%%
%\begin{align}
%\label{eq:parametric}
%\mathbf{S}_{\diamond}= \sum_{i = 0}^1 \sum_{j = 0}^1 s_{ij}  \left(\mathbf{S}_{T}^{i} \otimes  \mathbf{S}^{j}  \right)
%\end{align}
%
%where the four scalars $\{s_{ij}\}$ shape the formation of edges.
%For instance, setting only $s_{11} \neq 0$ we get the Kronecker product but allowing each $s_{ij}$ to take any real value we can weigh accordingly the impact of the spatial and temporal graphs into the final product graph. It should also be noted that $s_{00} \neq 0$ implies the presence of self-loops in the product graph. If all $s_{ij}$'s are non-zero, the parametric product graph has $|\ccalE_\diamond| = |\ccalE_\boxtimes|+NT$ edges, which are $NT$ more edges than the strong product because of these self-loops. 
Column-vectorizing $\bbX$ into $\bbx_\diamond =\operatorname{vec}(\bbX) \in \reals^{NT}$ we obtain a product graph signal in which the $i$th entry is the signal value at the spatiotemporal node $i_\diamond$. Some of such values are illustrated in Fig.~\ref{fig: product graph}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 						SECTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Problem Motivation}\label{subsec_probMotiv}

We are interested in learning representations from the spatiotemporal data in $\bbX$ for a particular task such as inferring the source of a signal~\cite{Zhao2020anomalydet}, forecasting future values~\cite{mo:yu2017spatio}, or classifying time series~\cite{mo:yan2018STGCNN}. While the product graph is a viable mathematical tool to represent the structure in $\bbX$, we can also ignore it and process $\bbX$ with standard approaches such as the vector autoregressive (VAR) models~\cite{lutkepohl2005new}, multilayer perceptrons (MLPs)~\cite{friedman2017elements}, or recurrent neural networks (RNNs)~\cite{rumelhart1986learning}. However, such techniques face two main limitations. First, their number of parameters and computational complexity is of order $\ccalO(N^2)$ as they involve dense layers, suffering the curse of dimensionality~\cite{bronstein2021geometric}. Second, they depend on the fixed order of the time series. The latter is a challenge because the learned representations do not permute with the time series and, when a new time series becomes available, the whole system needs to be retrained. Consequently, these models are not transferable.

One strategy to overcome such challenges is to exploit separately the spatial and the temporal structure by first processing $\bbX$ column-wise with a graph neural network (GNN)~\cite{GNNsurvey} and successively with a temporal convolution or RNN~\cite{mo:chai2018bike,mo:khodayar2018spatio}. However, such strategy fails to exploit the spatiotemporal coupling in the data and leverages only the coupling in the learned higher-level representation of the GNN, ultimately, limiting the performance and interpretability. One way to overcome this challenge is to embed a graph structure within a recursive model such as VAR~\cite{mo:isufi2019VARMA} or RNN~\cite{mo:seo2018GRNN,mo:ruiz2020gatedGRNN}. Working with graph-based VAR models is limiting because they work in the linear space, while graph-based RNN works only with a fixed latent-space dimension of $N$ (number of the nodes) or require an additional pooling step. Both the latter are uncomfortable because RNN-type of algorithms work best with a lower-dimensional latent space and finding the appropriate pooling strategy adds an extra challenge to the whole system~\cite{GNNsurvey}. Another aspect of RNNs is that they suffer training issues in their vanilla form; hence, LSTMs~\cite{hochreiter1997long} or GRUs~\cite{cho2014learning} are needed, which put more emphasis on the temporal dependencies rather than on the joint spatiotemporal ones.

Differently, we propose a first-principle neural network solution that exploits product graphs as an inductive bias for the spatiotemproal coupling, that is modular to any pooling technique, and that puts equal emphasis on the joint spatiotemporal learning. Building on first principles allows for a mathematical tractability akin to that of the principled spatial CNN~\cite{gama2020elvinmagazine}. To achieve these goals, we leverage the shift-and-sum principle of the convolution operation~\cite{oppenheim1999discrete} to propagate information over the product graph but differently from a GCNN~\cite{gama2020elvinmagazine} we leverage the sparsity of the product graph to handle its large dimensionality. Working with the convolution principle allows also developing an architecture that is equivariant to permutations~\cite{gama2020elvinmagazine}, enjoys a spectral analysis via the graph-time Fourier transform~\cite{grassi2017time,elvin2dfilters} (Section~\ref{sec_gtcnn}), and that is stable to perturbations in the spatial support (Section~\ref{sec_stability}).
%Besides the mathematical tractability, this principled solution compares well with existing alternatives in benchmark settings.


%\blue{Consider the data matrix $\bbX = [\bbx_1, \dots, \bbx_T]$ is a multivariate time-series, i.e, each row of $\bbX$ is a scalar time-series, and there are dependencies among them.
%Having a multivariate time-series data set such as $\ccalT = \{\bbX_i,\ccalY_i\}_{i=1}^m$, the goal is to find a mapping $\Phi(\cdot)$ to assign the input $\bbX$ to its desired output $\ccalY$, which implies both spatial and temporal relations encoded in $\bbS$ and $\bbS_T$.
%To learn a latent representation space for $\bbX$, conventional methods such as multi-layer perceptron or recurrent neural network are inefficient since they do not account for both spatial and temporal structure of data and the coupling between time and space.}
%
%\blue{We are interested in learning for $\bbx_t$'s that has an underlying graph structure, so we will develop a solution for it.
%Assume both spatial and temporal relations are given through graph shift operators $\bbS$ and $\bbS_T$, respectively.
%Consider graph-time signal $\bbx_\diamond = \text{vec}(\bbX)$ over the parametric product graph
%$\ccalG_\diamond = \ccalG_T \diamond \ccalG$.
%Hence, one such solution is to build a graph convolutional neural network as we have a graph $\ccalG_\diamond$ and a graph signal $\bbx_{\diamond}$.
%However, now we are working on a product graph that has some aspects which needs to be taken into account since the product graph is not an arbitrary graph.
%In upcoming sections, our focus will be on implementing and analyzing graph-time neural networks, and processing multivariate time-series with them.} \red{EI: (i) check the new problem motivation I wrote and if there is something in this blue part worth mentioning. (ii) check the problem motivation again as we need to reduce the first two paragraphs. They are too long.}

%Consider an $N \times 1$ multivariate signal $\bbx_t$ collected over $T$ time instances in matrix $\bbX = [\bbx_1, \ldots, \bbx_T ]$, such as sensor recordings in a
%sensor network.
%Each row of $\bbX$, $x_t(i)$, indicates a scalar time-series with its own temporal patterns.
%Meanwhile, each column, $\bbx_t$, represents a graph signal over the network at a certain instant which stands for spatial dependencies in the data.
%So, the data $\bbX$ has combined spatiotemporal relations governing on both time and space at the same time.
%From $\bbX$, we want to learn representations for any arbitrary task such as detecting the source of a diffusion process, forecasting, or anomaly detection.
%Although both temporal and spatial relations play an important role in processing such data, there are spatiotemporal relations in $\bbX$, which
%if fully-exploited serve as a powerful inductive bias to learn representations~\cite{battaglia2018inductivebias}.

%When signal $\bbx_t$ has an (hidden) underlying structure, we
%can represent its \textit{spatial} relations through a spatial graph $\ccalG = (\ccalV, \ccalE)$ of
%$N$ nodes in set $\ccalV = \{1, \ldots , N\}$ and $|\ccalE|$ edges in set $\ccalE \subseteq \ccalV \times \ccalV$. Signal
%$\bbx_t = [x_t(1), . . . , x_t(N) ]^\top$
%is a collection of scalars $x_t(i)$ residing on node $i$
%at time $t$. Likewise, we can capture the \textit{temporal} relations by viewing
%each row $\bbx^i = [x_1(i), \ldots, x_T(i)]^\top$ of $\bbX$ as a graph signal over the nodes
%of a temporal graph $\ccalG_T = (\ccalV_T , \ccalE_T )$ of $T$ nodes $\ccalV_T = \{1, \ldots, T\}$
%and $|\ccalE_T |$ edges $\ccalE_T = (t, t^\prime)$. Set $\ccalE_T$ contains an edge if signals at
%time instances $t$ and $t^\prime$ are related.
%Examples for $\ccalG_T$ are the directed line graph that assumes signal $x_t(i)$ depends only on the former instance
%$x_{t-1}(i)$, the cyclic graph that accounts for periodicity, or any other graph
%that encodes the temporal dependencies in $\bbX$, see Fig.~\ref{fig: signal over graphs}. We represent
%graphs $\ccalG$ and $\ccalG_T$ through their respective graph shift operator matrices
%$\bbS \in \reals^{N \times N}$ and $\bbS_T \in \reals^{T \times T}$.
%These matrices can be either Laplacian, adjacency, or any variants of them~\cite{sandryhaila2013discrete}.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% FIGURE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}
%	\begin{center}
%		\includegraphics[width=0.7\linewidth]{Figures/Fig1}
%	\end{center}
%	\caption{(a) Indicates the graph signal at time instant $t$ over the spatial graph. (b) Illustrates the time-series over temporal graph. (green) directed line graph, (green and grey) cyclic graph.}
%	\label{fig: signal over graphs}	
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Given graphs $\ccalG$ and $\ccalG_T$ , we can capture the spatio-temporal relations in $\bbX$ through the product graph:  %
%\begin{equation}
%\mathcal{G}_{\diamond}=   \mathcal{G}_{T}   \diamond \mathcal{G} =\left(\mathcal{V}_{\diamond}, \mathcal{E}_{\diamond} ,\mathbf{S}_{\diamond}\right),
%\end{equation}
%%
%where the node set $\ccalV_\diamond= \ccalV_T \times \ccalV$ is the Cartesian product between $\ccalV_T$ and $\ccalV$ ( hence of cardinality $|\mathcal{V}_{\diamond}|=NT$), the edge set $\ccalE_\diamond \subseteq \mathcal{V}_\diamond \times \mathcal{V}_\diamond$, and the shift operator $\bbS_\diamond \in \reals ^{NT \times NT}$ are dictated by the type of product graph.
%Product graphs are the Kronecker, Cartesian, and strong product \cite{sandryhaila2014big, grassi2017time}, defined as:
%%%%%%%%%%%%%%%%%%
%\begin{itemize}
%	\item \textit{Kronecker product}: $G_{\otimes} = G_T {\otimes} G = (V_{\otimes}, E_\otimes, S_\otimes)$. The edge set is $\ccalE_{\otimes} = \ccalE_T \otimes \ccalE$ with cardinality of $|\ccalE_\otimes| = 2|\ccalE| |\ccalE_T|$. The graph shift operator is $\bbS_{\otimes}=\bbS_T \otimes \bbS$.
%	
%	\item \textit{Cartesian product}: $G_{\times} = G_T {\times} G = (V_{\times}, E_\times, S_\times)$.  The edge set is \blue{$\ccalE_\times = \ccalE_T \otimes \mathbf{I}_N + \mathbf{I}_T \otimes \ccalE$}\red{EI: this blue part does not make sense, you cannot mix sets with matrices.} with cardinality of $|\ccalE_\times| = T|\ccalE| + N|\ccalE_T|$.
%	The graph shift operator is $\mathbf{S}_{ \times}=\mathbf{S}_T \otimes \mathbf{I}_{N}+\mathbf{I}_{T} \otimes \mathbf{S}$.
%	
%	\item \textit{Strong product}: $G_{\boxtimes} = G_T {\boxtimes} G = (V_{\boxtimes}, E_\boxtimes, S_\boxtimes)$.
%	The edge set is with $\ccalE_\boxtimes = \ccalE_\otimes + \ccalE_\times$ cardinality of $|\ccalE_\boxtimes| = |\ccalE| |\ccalE_T| + T|\ccalE| + N|\ccalE_T|$.
%	The graph shift operator is $\bbS_{\boxtimes}=\mathbf{S}_T \otimes \mathbf{I}_{N}+\mathbf{I}_{T} \otimes \mathbf{S} + \bbS_T \otimes \bbS$.
%\end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%Fig.~\ref{fig: product graph} illustrates all these product graphs.
%\begin{figure}
%	\begin{center}
%		\includegraphics[width=0.7\linewidth]{Figures/Fig2}
%	\end{center}
%	\caption{Product graphs. (grey edges) Kronecker product. (green and red) Cartesian product. (All edges) Strong product. \red{EI: make the caption longer, add some signals over the nodes as you do in the othr figure (maybe don't add them for the middle spatial graph in the PG plot), also make this bigger and trim white spaces around.}}
%	\label{fig: product graph}
%\end{figure}

%All the aforementioned product graphs can be generalized through a parametric model, called parametric product graph \cite{natali2020forecasting}, with shift operator:
%%
%\begin{align}
%\label{eq:parametric}
%\mathbf{S}_{\diamond}= \sum_{i = 0}^1 \sum_{j = 0}^1 s_{ij}  \left(\mathbf{S}_{T}^{i} \otimes  \mathbf{S}^{j}  \right),
%\end{align}
%where $\{s_{ij}\}$ are scalars that shape the formation of the edges. The parametric product graph captures the spatio-temporal coupling with the four scalars $s_{ij}$ . If all $s_{ij}$'s are non-zero, the parametric
%product graph has $|\ccalE_\diamond| = |\ccalE_\boxtimes|+NT$ edges, which are $NT$ more edges
%than the strong product because of self-loops ($s_{00} \neq 0)$.
%Column-vectorizing $\bbX$ yields a product graph signal $\bbx_\diamond =
%\operatorname{vec}(\bbX) \in \reals^{NT}$ in which node $i_\diamond \in \ccalV_\diamond$ represents the space-time
%location $(i, t)$ with signal value $x_t(i)$, i.e., the $i_\diamond$th entry of $\bbx_\diamond$.
%Our goal is to exploit the coupling product graph signal–product graph to learn spatiotemporal representations in a form akin to temporal or graph convolutional neural networks.

%
%
%\subsection{Problem Definition}
%
%Consider the data matrix $\bbX = [\bbx_1, \dots, \bbx_T]$ is a multivariate time-series, i.e, each row of $\bbX$ is a scalar time-series, and there are dependencies among them.
%Having a multivariate time-series data set such as $\ccalT = \{\bbX_i,\ccalY_i\}_{i=1}^m$, the goal is to find a mapping $\Phi(\cdot)$ to assign the input $\bbX$ to its desired output $\ccalY$, which implies both spatial and temporal relations encoded in $\bbS$ and $\bbS_T$.
%To learn a latent representation space for $\bbX$, conventional methods such as multi-layer perceptron or recurrent neural network are inefficient since they do not account for both spatial and temporal structure of data and the coupling between time and space.
%
%We are interested in learning for $\bbx_t$'s that has an underlying graph structure, so we will develop a solution for it.
%Assume both spatial and temporal relations are given through graph shift operators $\bbS$ and $\bbS_T$, respectively.
%Consider graph-time signal $\bbx_\diamond = \text{vec}(\bbX)$ over the parametric product graph
%$\ccalG_\diamond = \ccalG_T \diamond \ccalG$.
%Hence, one such solution is to build a graph convolutional neural network as we have a graph $\ccalG_\diamond$ and a graph signal $\bbx_{\diamond}$.
%However, now we are working on a product graph that has some aspects which needs to be taken into account since the product graph is not an arbitrary graph.
%In upcoming sections, our focus will be on implementing and analyzing graph-time neural networks, and processing multivariate time-series with them.


==> GTCNN paper/Sections/Conclusion.tex <==
We introduced graph-time convolutional neural networks as a model to learn from spatiotemporal data.
The GTCNN uses product graph to convert dynamic data over network into static data over a larger graph.
Afterward, a shift-and-sum convolution mechanism conveys the information over the product graph to exploit spatiotemporal dependencies in the data.
The product graph itself can also be parametric to enable the model to learn temporal relationships directly from data, and also allows us to implement the GTCNN recursively and avoid storing and processing large graphs.
We proposed a spectral domain analysis for graph-time convolutional filters and showed they operate as point-wise multiplication between the filters frequency response and the time series graph-time Fourier transform. Such a spectral analysis allowed us to study the stability of the GTCNN to perturbations in the spatial support.
We showed that the GTCNN becomes linearly less stable as the time series length increases.
However, it is yet more stable than the case where we consider time as distinct features and approach the problem via GCNNs.
The numerical results also approved that GTCNNs performs better than a baseline GCNN model.
Moreover, GTCNN compares well on benchmark datasets to state-of-the-art graph-based models but it suffered to capture long term patterns in the data.
This is because the GTCNN works with large graphs and cannot maintain long input time series.
The presented recursive model overcomes the memory consumption problem for large graphs and long time series while computational complexity needs to be improved yet as a direction for future works. 


==> GTCNN paper/Sections/GTCNNsec.tex <==










In this section, we define the graph-time convolutional neural network (GTCNN) and discuss its properties both in the vertex and in the spectral domain.


%====================================================================================================================================================================================%
%====================================================================================================================================================================================%
% 		SUBSECTION
%====================================================================================================================================================================================%
%====================================================================================================================================================================================%


\subsection{Graph-Time Convolutional Filters}\label{subsec_gtcf}

\begin{figure*}[!t]
	\centering
	\input{Figures/GT_Filter/gtfilter_kron}
	\caption{Graph time convolutional filter of order two illustrated for a Cartesian product graph.
		Each block shifts the signal $\bbx_\diamond$ over the product graph by its graph shift operator $\bbS_\diamond$. Each shift implies a neighborhood coverage highlighted in yellow for a particular node. Each shifted signal $\bbS_\diamond^k \bbx_{\diamond}$ is scaled by its filter coefficient $h_k$ and summed up to build the output $\bby_{\diamond}$. Changing the product graph implies a different spatiotemporal neighborhood coverage.}
	\label{fig:gt_filter}
\end{figure*}

The key element to build a GTCNN is the \emph{graph-time convolutional filter}. For a product graph $\ccalG_\diamond = (\ccalV_\diamond,\ccalE_\diamond,\bbS_\diamond)$ and signal $\bbx_\diamond$, the output $\bby_\diamond$ of a graph-time convolutional filter of order $K$ is
%
\begin{equation}\label{eq:graphtimefilter}
\bby_\diamond = \bbH(\bbS_\diamond)\bbx_\diamond = \sum_{k=0}^K h_k \bbS_\diamond^k \bbx_\diamond
\end{equation}
%
where $h_0,\dots,h_K$ are the parameters and $ \bbH(\bbS_\diamond):= \sum_{k=0}^K h_k \bbS_\diamond^k$ denotes the filtering matrix. The qualifier convolution for filter \eqref{eq:graphtimefilter} comes from the fact that it shifts the input $\bbx_\diamond$ up to $K$ times over the product graph $\bbS_\diamond^0\bbx_\diamond, \bbS_\diamond^1\bbx_\diamond, \ldots, \bbS_\diamond^K\bbx_\diamond$ and builds the output $\bby_\diamond$ as a scaled sum of these shifts; see Fig.~\ref{fig:gt_filter}. Since $\bbS_\diamond$ is spatiotemporally local, the shift $\bbS_\diamond\bbx_\diamond$ diffuses the signal from the spatiotemporal node $i_\diamond$ to any other immediate spatiotemporal neighbor $j_\diamond$. From recursion $\bbS_\diamond^k\bbx_\diamond = \bbS_\diamond(\bbS_\diamond^{k-1}\bbx_\diamond)$, we can see that higher-order powers $\bbS_\diamond^k$ diffuse the signal to spatiotemporal neighbors that up to $k-$hops. This implies that filter \eqref{eq:graphtimefilter} is spatiotemporally local in a neighborhood of radius $K$. The filter resolution depends on the order $K$ but also on the type of product graph. For instance, the Kronecker product ignores the information present at time $t$ limiting the spatial resolution but has a high temporal one; the Cartesian product brings in the spatial information of time $t$ but accounts for the temporal proximity only for signal values at the same node; the strong product accounts for both and needs a lower order $K$ to cover a particular neighborhood; Fig.~\ref{fig:gt_filter}. 
%The parametric product graph adopts the resolution through coefficients $\{s_{ij}\}$.

The locality of $\bbS_\diamond$ allows obtaining the output $\bby_\diamond$ in~\eqref{eq:graphtimefilter} with a computational cost of order $\ccalO(K|\ccalE_\diamond|)$. The latter can be achieved by leveraging the recursion $\bbS_\diamond^k\bbx_\diamond= \bbS_\diamond(\bbS_\diamond^{k-1}\bbx_\diamond)$. This complexity order is appealing despite we work with a large GSO and input vector. However, it should be noted that $|\ccalE_\diamond|$ is in turn governed by the type of product graph [cf. Fig.~\ref{fig: product graph}], thus making the strong product a suitable choice only if the spatial graph is highly sparse. It also follows from~\eqref{eq:graphtimefilter} that the order of parameters is $\ccalO(K)$ and it is independent on the spatial and temporal dimensions.

%In this section we propose GTCNNs and discuss their implementation aspects.
%We will also provide a frequency analysis for the graph-time convolutional filters used in this model, which we will use to theoretically analyze such models.

%====================================================================================================================================================================================%
%====================================================================================================================================================================================%
%====================================================================================================================================================================================%

%\subsection{Graph-Time Convolutional Filters}
%Consider graph-time signal $\bbx_\diamond$ over the parametric product graph
%$\ccalG_\diamond = \ccalG_T \diamond \ccalG$,
%where $\ccalG_T = (\ccalV_T,\ccalE_T)$ and $\ccalG=(\ccalV,\ccalE)$ are the temporal and spatial graphs, respectively.
%So, we can define the \emph{graph-time convolutional filter} as 
%\begin{equation}
%\bby_\diamond = \bbH(\bbS_\diamond)\bbx_\diamond
% = \sum_{k=0}^K h_k \bbS_\diamond^k \bbx_\diamond
%% = \sum_{k=0}^K h_k \left(
%%\sum_{i=0}^1 \sum_{j=0}^1 s_{ij} (\bbS_T^i \otimes \bbS^j)
%%\right)^k \bbx_\diamond,
%\label{eq:graphtimefilter}
%\end{equation}
%where $\bbS_\diamond$ is the parametric product graph in~(\ref{eq:parametric}), and $\bbH(\bbS_\diamond) = \sum_{k=0}^K h_k \bbS_\diamond^k$ indicates the graph-time convolutional filter with coefficients $h_k$.
%The graph-time convolutional filter in~(\ref{eq:graphtimegeneralfilter}) consists of $K$ shift-and-sum of the input signal over product graph which is similar to conventional convolutional filters.
%Assume nodes $i$ and $j$ are adjacent in the spatial graph $\ccalG$.
%When we use product graph $\ccalG_\diamond = \ccalG_T \diamond \ccalG$, the previous value of time-series over node $j$, i.e., $x_{t-1}(j)$, will be in the neighborhood of node $i$. 
%Now, by shifting the input signal, the information propagates over the product graph, which means the nodes pass their values through both time and space according to parameters $s_{ij}$.
%This new neighborhoods allow graph-time convolutional filters to exploit spatiotemporal patterns and become a promising tool for processing multivariate time-series.
 
%When we product the graphs, the spatial graph replicates $T$ times over the time dimension, and the choice of $s_{ij}$ and $\bbS_T$ determine the structure of the product graph.

%\begin{figure}[t]
%	\centering
%	\includegraphics[width = 0.7\linewidth]{Figures/productgraph.png}
%	\caption{
%		Product graphs.
%		Kronecker product has the gray edges.
%		Cartesian has the red and green edges.
%		Strong product has all the red, gray, and green edges.
%		Parametric product has all the edges and also self loops if all $s_{ij} \neq 0$.
%		Adopted from~\cite{mo:isufi2021graphproduct}.
%	}
%	\label{fig:productgraph}
%\end{figure}

%====================================================================================================================================================================================%
%====================================================================================================================================================================================%
% 		SUBSECTION
%====================================================================================================================================================================================%
%====================================================================================================================================================================================%
\subsection{GTCNNs}\label{subsec_gtcnn}

A graph-time convolutional neural network (GTCNN) is a composition of graph-time convolutional filters with pointwise nonlinearities. Specifically, consider an architecture composed of $L$ layers $\ell = 1, \ldots, L$ and let $\bbH_\ell(\bbS_\diamond) = \sum_{k=0}^K h_{k\ell} \bbS_\diamond^k$ be the filter used at layer $\ell$.
The GTCNN propagation rule is
%
\begin{equation}
\bbx_{\diamond,\ell} = \sigma \big( \bbH_\ell(\bbS_\diamond)\bbx_{\diamond,\ell-1}		\big) = \left(\sum_{k=0}^K h_{k\ell} \bbS_\diamond^k\bbx_{\diamond,\ell-1}		\right)
\end{equation}
%
where $\bbx_{\diamond,0}\coloneqq\bbx_\diamond$ is the GTCNN input. Fig.~\ref{fig:GTCNN_bd} illustrates a GTCNN of three layers. To augment the representation power, we consider multiple nodal features per layer in matrix $\bbX_{\diamond,\ell-1} = [\bbx_{\diamond,\ell-1}^1, \ldots, \bbx_{\diamond,\ell-1}^F] \in \reals^{NT \times F}$ where each column $\bbx_{\diamond,\ell-1}^g$ is a graph-time signal feature at layer $\ell-1$. These features are passed through a bank of graph-time convolutional filters and pointwise nonlinearities to yield the output features of layer $\ell$
%
\begin{equation}\label{eq.filter_bankMat}
\bbX_{\diamond,\ell} = \sigma\left(\sum_{k=0}^K \bbS_\diamond^k\bbX_{\diamond,\ell-1}\bbH_{k\ell}	\right)
\end{equation}
%
where $\bbH_{k\ell} \in \reals ^{F \times F}$ is the parameter matrix containing the coefficients of the filter bank at layer $\ell$. To ease the analysis of the filer bank in \eqref{eq.filter_bankMat}, we make explicit the input-output relation between the $f$th output feature $\bbx_{\diamond,\ell}^f$ and the $g$th input feature $\bbx_{\diamond,\ell-1}^g$ as
%
\begin{equation}\label{eq.eq.filter_bank}
\bbx_{\diamond,\ell}^f = \sigma \bigg(\sum_{g = 1}^F \bbH_\ell^{fg}(\bbS_\diamond)\bbx_{\diamond,\ell-1}^g	\bigg) = \sigma \bigg(	\sum_{g = 1}^F	\sum_{k=0}^K h_{k\ell}^{fg}\bbS_\diamond^k\bbx_{\diamond,\ell-1}^g	\bigg)
\end{equation}
%
for all $f = 1, \ldots, F$ and where $\bbH_\ell^{fg}(\bbS_\diamond) = \sum_{k=0}^K h_{k\ell}^{fg}\bbS_\diamond^k$ is one of the $F^2$ filters used in layer $\ell$.

Recursions \eqref{eq.filter_bankMat} (resp. \eqref{eq.eq.filter_bank}) are repeated for all layers. In the last layer $\ell = L$, we consider without loss of generality the number of output features is one, i.e., $\bbx_{\diamond,L} := \bbx_{\diamond,L}^1$. This output is a function of the input $\bbx_\diamond$ and the collection of all filter banks $\bbH_\ell^{fg}(\bbS_\diamond)$ [cf. \eqref{eq:graphtimefilter}]. Grouping all filters in the filter tensor $\ccalH(\bbS_\diamond) = \{	\bbH_\ell^{fg}(\bbS_\diamond)	\}_{\ell fg}$, we can define the GTCNN output as the mapping
%
\begin{equation}\label{eq:GTCNN}
\bbx_{\diamond,L}:= \Phi(\bbx_\diamond;\ccalH(\bbS_\diamond))\quad \text{with}\quad \ccalH(\bbS_\diamond) = \{	\bbH_\ell^{fg}(\bbS_\diamond)	\}_{\ell fg}.
\end{equation}
%
%Fig.~\ref{fig:GTCNN_bd} illustrates a GTCNN with three layers.
The GTCNN parameters are learned to minimize a loss $\ccalL(\bbx_L, \bbY)$ computed over a training set of input-output pairs $\ccalT = \{\bbx_\diamond, \bbY\}$.
%where $\ccalX$ is the representation space of the input and $\ccalY$ that of the output. 

As it follows from \eqref{eq:graphtimefilter}, the number of parameters in each filter is $K+1$. This gets scaled by the number of filters per layer $F^2$ and the number of layers $L$, yielding an order of $\ccalO(KF^2L)$ parameters defining the GTCNN. Likewise, the computational complexity for running the filter bank for $L$ layers is of order $\ccalO(KF^2L|\ccalE_\diamond|)$. Such orders are similar to those of conventional GCNNs working with time invariant signals. This is a consequence of exploiting the sparsity of product graphs and the spatiotemporal coupling via graph convolutional filters [cf. \eqref{eq:graphtimefilter}]. In the next section, we shall discuss how to \emph{learn} this spatiotemporal coupling.


%To discuss computational aspects of GTCNNs, we need to consider two separate cases; fixed product graph and learnable product graph.
%If the product graph is fixed, $\bbS_\diamond$ has a sparsity of order
%$| \ccalE_\diamond | = NT + N | \ccalE_T | + T | \ccalE | + | \ccalE_T | | \ccalE |$.
%Although we are working with much bigger graphs in GTCNNs, one should notice that the product graph is too sparse.
%The shift operator $\bbS_\diamond\bbx_\diamond$ has a cost of $\ccalO((NT)^2)$, but due to the sparsity of $\bbS_\diamond$ it can be computed by the number of edges $\ccalO(| \ccalE_\diamond |)$.
%Computing output $\bby_\diamond$ requires computing the shifts
%$\bbx_\diamond^{(k)} = \bbS_\diamond^k\bbx_\diamond$ which has the huge computational cost of $\ccalO(K(NT)^3)$.
%For this, we can use the well-known recursive implementation of shifting signals over a graph~\cite{isufi2016armagraph} and write
%$\bbx_\diamond^{(k)} = \bbS_\diamond^k\bbx_\diamond = \bbS_\diamond \bbx_\diamond^{(k-1)}$.
%Hence, thanks to the locality of shift operator $\bbS_\diamond$, we can obtain the output $\bby_\diamond$ with the linear cost $\ccalO(K|\ccalE_\diamond|)$.
%This cost will adds up to $\ccalO(F^2L(K+1)|\ccalE_\diamond|)$ for the whole GTCNN, assuming that all layers have $F$ features for the sake of simplicity, since graph-time convolution is a local operator over product graph.


%%%%%%%%%%%%%%%
% 		REMARK
\smallskip
\noindent
\textbf{Alternative graph-time neural networks.}
%
	Once the product graph is built, we can employ any aggregation scheme to collect spatiotemporal information. For the sake of completness, we detail here the message passing neural network (MPNN)~\cite{hamilton2017representation} and the graph attention network (GAT)~\cite{velivckovic2017graph}.
%	However, we focus on convolutional neural networks on this paper.

	\emph{MPNNs} update a spatiotemporal node's latent representation $\bbx_{\diamond,\ell}$ by passing a message from its neighborhood as
	\begin{equation}
		\bbm_{\diamond,\ell-1}^{(i)} = f(\bbx_{\diamond,\ell-1}[j]: (i,j)\in \ccalE_\diamond)
	\end{equation}
	where $\bbm_{\diamond,\ell-1}^{(i)}$ is the message vector for node $i$, $\bbx_{\diamond,\ell-1}[j]$ is the output of layer $\ell - 1$ at node $j$, and $f(\cdot)$ is a differentiable and permutation equivariant function.
	Each node's latent vector can be updated based on inferred messages and its current feature vector as
	\begin{equation}
		\bbx_{\diamond,\ell} = g(\bbx_{\diamond,\ell-1},\bbM_{\diamond,\ell-1})
	\end{equation}
	where $\bbM_{\diamond,\ell-1} = \{\bbm_{\diamond,\ell-1}^{(i)}\}$ collects all the messages for each node and $g(\cdot)$ is an arbitrary differentiable function (i.e., neural networks).
	Since we are considering the spatiotemporal product graph, the messages are including spatiotemporal information, and the type of product graph dictates which nodes are forwarding these messages.
	 
	\emph{GATs} use an attention mechanism to update latent representation of each node based on its neighborhood as
	%This can be expressed as:
	\begin{equation}
		\bbx_{\diamond,l+1}[i] = \sigma\left(\sum_{(i,j)\in\ccalE_\diamond} \alpha_{ij}\bbH\bbx_{\diamond,\ell}[j]\right)
	\end{equation}
	where $\alpha_{ij}$ indicates attention coefficients and $\bbH \in \reals^{F\times F}$ is a linear transformation to map the features between layers.
	The type of product graph rules the attention coefficients $\alpha_{ij}$ and their calculation.
	
	In both MPNN and GAT models, we can split the rule over space and time to have a different message passing or attention scheme.
	All in all, these represent different principles to learn spatiotemporal representation with product graphs. We continue with convolutional principle since it provides theoretical tools for their analysis and leave the MPNNs and GATs to interested readers.


\begin{figure}[!t]
	\centering
	\input{Figures/GTCNN_BD}
	\caption{GTCNN block diagram. On each layer a graph time convolutional filter [cf.~\eqref{eq:graphtimefilter}] is composed by a point-wise non-linearity, and all these layers are cascaded to generate the output.}
	\label{fig:GTCNN_bd}
\end{figure}
%
%
%\subsection{GTCNNs}
%Upon defining a product graph $\ccalG_\diamond$ and a product graph signal $\bbx_\diamond$, we can re-use the GCNN idea to develop a neural network over the product graph following the first principles of the convolution operation.
%A graph-time convolutional neural network (GTCNN) is a cascaded architecture of $L$ layers each having a graph-time convolutional filter and a point-wise nonlinearity.
%At layer $l$, we have a collection of $F$ graph signal features $\bbx_{\diamond,l-1}^g$ for $g = 1, \dots, F$ as the input.
%Each input feature $\bbx_{\diamond,l-1}^g$ is processed in parallel by a bank of $F_l$ graph-time filters $\bbH_l^{fg}(\bbS_\diamond)$ to yield the filtered features
%\begin{equation}
%\bbz_{\diamond,l}^{fg} = \bbH_l^{fg}(\bbS_\diamond)\bbx_{\diamond,l-1}^g
%\quad \text{for}
%\quad (f;g) = (1;1), \dots, (F;F).
%\end{equation}
%Filtered features $\bbz_{\diamond,l}^{fg}$ obtained from a common input $\bbx_{\diamond,l-1}^g$ are summed to form the higher-level linear features of layer $l$
%\begin{equation}
%\bbz_{\diamond,l}^{f} = \sum_{g=1}^{F} \bbz_{\diamond,l}^{fg} = \sum_{g=1}^{F} \bbH_l^{fg}(\bbS_\diamond)\bbx_{\diamond,l-1}^g
%\quad \text{for}
%\quad f = 1, \dots, F
%\label{eq:latent}
%\end{equation}
%which are a collection of $F$ graph signal features.
%Now, these higher-level linear features are passed to a point-wise nonlinearity to produce a collection of $F_l$ higher-level nonlinear features $\bbx_{\diamond,l}^f$ which constitute the output of layer $l$,
%\begin{equation}
%\bbx_{\diamond,l}^f = \sigma_l(\bbz_{\diamond,l}^{f})
%\quad \text{for}
%\quad f = 1, \dots, F_l
%\end{equation}
%where $\sigma(\cdot)$ is the nonlinearity.
%
%In the last layer $l = L$, we assume there is a single feature signal $F_L = 1$, which we consider the output of the GTCNN.
%We write this output compactly as
%\begin{equation}
%\Phi(\bbx_\diamond;\bbS_\diamond;\ccalH) = \sigma_L \left(
%\sum_{g=1}^{F} \bbH_L^{fg}(\bbS_\diamond)\bbx_{\diamond,L-1}^g
%\right)
%\end{equation}
%to specify the dependence from the product graph $\bbS_\diamond$, graph-time signal $\bbx_\diamond$, and parameters set $\ccalH$ defining all graph-time filters in~(\ref{eq:latent}).
%
%%====================================================================================================================================================================================%
%%====================================================================================================================================================================================%
%%====================================================================================================================================================================================%
%
%To discuss computational aspects of GTCNNs, we need to consider two separate cases; fixed product graph and learnable product graph.
%If the product graph is fixed, $\bbS_\diamond$ has a sparsity of order
%$| \ccalE_\diamond | = NT + N | \ccalE_T | + T | \ccalE | + | \ccalE_T | | \ccalE |$.
%Although we are working with much bigger graphs in GTCNNs, one should notice that the product graph is too sparse.
%The shift operator $\bbS_\diamond\bbx_\diamond$ has a cost of $\ccalO((NT)^2)$, but due to the sparsity of $\bbS_\diamond$ it can be computed by the number of edges $\ccalO(| \ccalE_\diamond |)$.
%Computing output $\bby_\diamond$ requires computing the shifts
%$\bbx_\diamond^{(k)} = \bbS_\diamond^k\bbx_\diamond$ which has the huge computational cost of $\ccalO(K(NT)^3)$.
%For this, we can use the well-known recursive implementation of shifting signals over a graph~\cite{isufi2016armagraph} and write
%$\bbx_\diamond^{(k)} = \bbS_\diamond^k\bbx_\diamond = \bbS_\diamond \bbx_\diamond^{(k-1)}$.
%Hence, thanks to the locality of shift operator $\bbS_\diamond$, we can obtain the output $\bby_\diamond$ with the linear cost $\ccalO(K|\ccalE_\diamond|)$.
%This cost will adds up to $\ccalO(F^2L(K+1)|\ccalE_\diamond|)$ for the whole GTCNN, assuming that all layers have $F$ features for the sake of simplicity, since graph-time convolution is a local operator over product graph.

%====================================================================================================================================================================================%
%====================================================================================================================================================================================%
% 		SUBSECTION
%====================================================================================================================================================================================%
%====================================================================================================================================================================================%

\subsection{Learning the Spatiotemporal Coupling}\label{subsec_learnSpatioTemp}

The GTCNN output in \eqref{eq:GTCNN} is influenced by the type of product graph but it is unclear which form is most suitable for a specific problem. To avoid imposing a wrong inductive bias, we consider the parametric product graph GSO
%
\begin{align}
\label{eq:generalgtfilter}
\mathbf{S}_{\diamond}= \sum_{i = 0}^1 \sum_{j = 0}^1 s_{ij}  \left(\mathbf{S}_{T}^{i} \otimes  \mathbf{S}^{j}  \right)
\end{align}
%
where by learning the four scalars $\{s_{ij}\}$ we learn the spatiotemporal coupling. The parametric product graph generalizes the three product graphs seen in Section~\ref{subsec_PG}. For instance, setting $s_{11}=1$ and the rest zero we get the Kronecker product. But allowing each $s_{ij}$ to take any real value weigh accordingly the impact of the spatial and temporal graphs into the final product graph. Note also that $s_{00} \neq 0$ implies the presence of spatiotemporal self-loops. If all $s_{ij}$'s are non-zero, the parametric product graph has $|\ccalE_\diamond| = |\ccalE_\boxtimes|+NT$ edges, which are $NT$ more edges than the strong product because of these self-loops. 

Building a GTCNN with the graph-time convolutional filter~\eqref{eq:graphtimefilter} but with the GSO~\eqref{eq:generalgtfilter} matches the spatiotemporal coupling with the task at hand. However, treating $\{s_{ij}\}$ as learnable parameters is practical only if we fix the filter order to $K = 1$.\footnote{This would be the spatiotemporal form of GCN~\cite{GCN_Welling}.}
For higher orders $K \ge 2$ this implies pre-computing the powers $\mathbf{S}_{\diamond}^k$ of~\eqref{eq:generalgtfilter} and storing them in the memory as the computational complexity of each multiplication is of order $\ccalO((NT)^3)$.
Yet, storing the powers in the memory is still impractical for large spatial graphs.
Another way to mitigate these issues is to rearrange the whole filter expression as shown next.

%%%%%%%%%%%%%%%
% PROPOSITION
\begin{proposition}
	\label{prop1}
	Consider the spatial graph $\ccalG$ with shift operator $\bbS$ and the temporal graph $\ccalG_T$ with shift operator $\bbS_T$. The graph-time convolutional filter in~\eqref{eq:graphtimefilter} operating with the parametric product graph in~\eqref{eq:generalgtfilter} is a particular case of
%
	\begin{equation}
	\bbH(\bbS,\bbS_T) =
	\sum_{k=0}^{\bar{K}}
	\sum_{l=0}^{\tilde{K}}
	h_{kl} (\bbS_T^l \otimes \bbS^k)
	\label{eq:graphtimegeneralfilter}
	\end{equation}
%	
where $\bar{K}$ and $\tilde{K}$ are the orders over the spatial and temporal graphs respectively and $\{h_{kl}\}$ are the parameters.
\end{proposition}
%
\begin{proof}
	See Appendix~\ref{sec:gtfilter_proof}.
\end{proof}

Building a GTCNN with a filter tensor $\ccalH(\bbS, \bbS_T) = \{	\bbH_\ell^{fg}(\bbS,\bbS_T)	\}_{\ell fg}$ yields an architecture that is more flexible than \eqref{eq:GTCNN}. This is because of:
%
\begin{enumerate}
%
\item Filter $\bbH(\bbS,\bbS_T)$ [cf. \eqref{eq:graphtimegeneralfilter}] has more freedom to control the spatial and temporal resolution in each layer through orders $\bar{K}$ and $\tilde{K}$. Differently, filter $\bbH(\bbS_\diamond)$ [cf. \eqref{eq:graphtimefilter}] does not allow for such an independent control, in which order $K$ influences the spatiotemporal resolution in a coupled manner. This allows exploiting more resolution in a particular domain.
%
\smallskip
%
\item Filter $\bbH(\bbS,\bbS_T)$ learns how the spatiotemporal coupling influences the graph-time convolution through parameters $\{h_{kl}\}$. This happens for each layer and feature. This is also more powerful than learning $\{s_{ij}\}$ and $\{h_k\}$ disjointly as in $\bbH(\bbS_\diamond)$ because it matches the importance of the multihop resolutions with the spatiotemporal links.
%
\smallskip
%
\item Filter $\bbH(\bbS,\bbS_T)$ enjoys the same computational cost of $\bbH(\bbS_\diamond)$. Computing the output $\bby_\diamond = \bbH(\bbS,\bbS_T)\bbx_\diamond$ requires computing all shifts $\bbx_\diamond^{(k,l)} = (\bbS_T^l \otimes \bbS^k) \bbx_\diamond$ for all $k\in [\bar{K}]$ and $l\in [\tilde{K}]$.
These shifts can be written in a recursive manner as
\begin{equation}
	\bbx_\diamond^{(k,l)} = (\bbS_T \bbS_T^{l-1} \otimes \bbS \bbS^{k-1}) \bbx_\diamond.
\end{equation}
Exploiting the properties of the Kronecker product\footnote{$(\bbA \otimes \mathbf{B})(\mathbf{C} \otimes \mathbf{D}) = \bbA \mathbf{C} \otimes \mathbf{B}\mathbf{D}$~\cite{petersen2008matrix}.}, we can write the latter as
%
\begin{align}
\bbx_\diamond^{(k,l)} &= (\bbS_T\otimes\bbS)(\bbS_T^{l-1} \otimes \bbS^{k-1})\bbx_\diamond \nonumber \\
&= (\bbS_T \otimes \bbI_N)(\bbI_T \otimes \bbS)(\bbS_T^{l-1} \otimes \bbS^{k-1})\bbx_\diamond.
\end{align}
%
Thus, we can compute $\bbx_\diamond^{(k,l)}$ recursively as
%
\begin{align}
\bbx_\diamond^{(k,l)} &=  (\bbS_T \otimes \bbI_N)\bbx_\diamond^{(k,l-1)}\nonumber\\
&= (\bbS_T \otimes \bbI_N)(\bbI_T \otimes \bbS)\bbx_\diamond^{(k-1,l-1)}
\label{eq:garphtimerecursion}
\end{align}
%
where $\bbx_\diamond^{(k,l-1)} = (\bbI_T \otimes \bbS)\bbx_\diamond^{(k-1,l-1)}$ is the spatially shifted signal and $\bbx_\diamond^{(0,0)} \coloneqq \bbx_\diamond$. Recursion~\eqref{eq:garphtimerecursion} implies that we can compute $\bbx_\diamond^{(k,l)}$ from $\bbx_\diamond^{(k-1,l-1)}$ with a cost of $\ccalO(T|\ccalE| + N|\ccalE_T|)$. Since we need to perform the latter for all $k\in [\bar{K}]$ and $l\in [\tilde{K}]$, we have a computational cost of order $\ccalO(\bar{K}T|\ccalE| + \tilde{K}N|\ccalE_T|)$, which is linear in the product graph dimension. The GTCNN cost is $F^2L$ times the latter.
\end{enumerate}
%

%If the parameters $\{s_{ij}\}$ are to be learned, computing $\bbS_\diamond$ beforehand or using~(\ref{eq:graphtimefilter}) can be unaffordable in large-scale settings since the powers of $\bbS_\diamond$ have cubic cost $\ccalO((NT)^3)$.
%To allow scalability, we first expand all polynomials of order $k$ and rearrange the terms to write~(\ref{eq:graphtimefilter}) as the following proposition.
%\begin{proposition}
%	The graph-time filter in~(\ref{eq:graphtimefilter}) can be transformed into
%	\begin{equation}
%	\bby_\diamond = \bbH(\bbS,\bbS_T) =
%	\sum_{k=0}^{\bar{K}}
%	\sum_{l=0}^{\tilde{K}}
%	h_{kl} (\bbS_T^l \otimes \bbS^k) \bbx_\diamond
%	\label{eq:graphtimegeneralfilter}
%	\end{equation}
%	for some orders $\bar{K}$ and $\tilde{K}$ and parameters $\{h_{kl}\}$.
%\end{proposition}
%\begin{proof}
%	See Appendix ?.
%\end{proof}
%The new form of graph-time filter in~(\ref{eq:graphtimegeneralfilter}) suggests two separate filter orders for spatial and temporal neighborhood which provides us with more control on the depth of the graph-time filter.
%In other words, each node in shifted signal $\bbx_\diamond^{(k,l)} = (\bbS_T^l \otimes \bbS^k) \bbx_\diamond$ gathers the information from $k$-hop neighborhood in spatial graph and $l$-hop neighborhood in temporal graph.
%
%To compute output $\bby_\diamond$, we need to compute all terms of the form
%$\bbx_\diamond^{(k,l)} = (\bbS_T^l \otimes \bbS^k) \bbx_\diamond$.
%Exploiting the Kronecker product property
%$(\bbA \otimes \mathbf{B})(\mathbf{C} \otimes \mathbf{D}) = \bbA \mathbf{C} \otimes \mathbf{B}\mathbf{D}$,
%we can write the latter as
%\begin{equation}
%\bbx_\diamond^{(k,l)} = (\bbS_T \otimes \bbI_N)(\bbI_T \otimes \bbS)(\bbS_T^{l-1} \otimes \bbS^{k-1})\bbx_\diamond.
%\end{equation}
%Thus, we can compute $\bbx_\diamond^{(k,l)}$ recursively again as
%\begin{align}
%\bbx_\diamond^{(k,l)} &= (\bbS_T \otimes \bbI_N)(\bbI_T \otimes \bbS)\bbx_\diamond^{(k-1,l-1)} \nonumber\\
%&= (\bbS_T \otimes \bbI_N)\bbx_\diamond^{(k,l-1)}
%\label{eq:garphtimerecursion}
%\end{align}
%with initialization $\bbx_\diamond^{(0,0)} = \bbx_\diamond$.
%Recursion~(\ref{eq:garphtimerecursion}) implies we can compute $\bbx_\diamond^{(k,l)}$ from $\bbx_\diamond^{(k-1,l-1)}$ with a cost of $\ccalO(T|\ccalE| + N|\ccalE_T|)$ and since we need to perform the latter for all $k\in [\bar{K}]$ and $l\in [\tilde{K}]$, we have a computational cost of
%$\ccalO(\bar{K}T|\ccalE| + \tilde{K}N|\ccalE_T|)$, which is linear in the product graph dimension.
%
%Note also that form~(\ref{eq:graphtimegeneralfilter}) improves our control on the spatiotemporal locality through orders $\bar{K}$ and $\tilde{K}$.
%A larger $\bar{K}$ implies more reach over the spatial graph, while a larger $\tilde{K}$ implies more reach over the temporal graph.
%Both orders are design choices.
%
%\footnote{\red{EI: for \eqref{eq:parametric}, we can analitically find what are the coefficients for a generic power $k$ and then use those for the GTCNN. We need to discuss this.}}
%====================================================================================================================================================================================%
%====================================================================================================================================================================================%
% 		SUBSECTION
%====================================================================================================================================================================================%
%====================================================================================================================================================================================%

\subsection{Properties}\label{subsec_prop}

The convolution principle allows studying two fundamental properties: equivariances to permutations in the vertex domain and the filters' frequency response in the frequency domain. We shall discuss these properties for a GTCNN with the more general filter $\bbH(\bbS,\bbS_T)$ [c.f.~\eqref{eq:graphtimegeneralfilter}] but the results hold also for filter $\bbH(\bbS_\diamond)$ [c.f.~\eqref{eq:graphtimefilter}].

\medskip
\noindent\textbf{Permutation equivariance}
allows assigning an arbitrary ordering to the nodes.
This is a desirable property since a graph does not change by the permutation of its nodes, hence the GTCNN output should stay unchanged up to a reordering.
%The advantage provided by permutation equivariancy is that the model can learn symmetries in the graph to aid learning process.
%Therefor, graph-time convolutional filters can exploit group symmetrical patterns in both temporal and spatial neighborhoods which plays an important role in the performance of GTCNNs.
The GTCNN is permutation equivariant as shown by the following proposition.
\begin{proposition}
	\label{prop2}
	Let $\bbx_\diamond = \textnormal{vec}(\bbX)$ be the signal over the product graph $\ccalG_\diamond$ with shift operator $\bbS_\diamond = \bbS_T \diamond \bbS$. Consider also the output of a graph-time filter $\bbH(\bbS_T,\bbS)\bbx_{\diamond}$. Then, for a permutation matrix $\bbP$ belonging to the set
	\begin{equation}
		\ccalP = \{\bbP = \{0,1\}^{N\times N} \colon \bbP\bbone=\bbone, \bbP^\top\bbone=\bbone\} \nonumber
	\end{equation}
	it holds that
	\begin{equation}
		\bbP\!^\top\!\textnormal{vec}\!^{-\!1}\!(\Phi(\bbx_\diamond;\ccalH(\bbS_T,\bbS)))\! =\!\Phi(\bbx_\diamond;\ccalH(\bbS_T,\bbP\!^\top\!\bbS\bbP))\textnormal{vec}(\bbP\!^\top\!\bbX).
	\end{equation}
\end{proposition}
\begin{proof}
	See Appendix.~\ref{sec:permequi_proof}.
\end{proof}


That is, the GTCNN operating on a multivariate time-series over a spatial graph $\bbS$ has the equally permuted output of the GTCNN operating on permuted spatial graph $\bbP^\top\bbS\bbP$.
This property allows the GTCNN to exploit the spatiotemporal data dependencies and symmetries encoded in the product graph to enhance learning~\cite{bronstein2021geometric}.
%Moreover, permutation equivariancy strengthen the model by enabling it to learn latent symmetries in the graph structure.


\medskip
\noindent\textbf{Spectral analysis}
of filter \eqref{eq:graphtimegeneralfilter} can help us to study their behaviors and what spectral features they learn for a specific task.
It also provides a fundamental framework for further analyzing the robustness of the GTCNNs to perturbations as we shall detail in the next section.
%In the next section, we shall use this frequency analysis to study the stability of GTCNN to perturbations in the spatial graph.
To do so, consider the eigendecomposition of the spatial GSO $\bbS= \bbV \bbLambda \bbV^{\herm}$ with eigenvevtors $\bbV = [\bbv_1, \ldots, \bbv_N]$ and eigenvalues $\bbLambda = \diag(\lambda_1,\dots,\lambda_N)$.
Consider also the eigendecomposition of the temporal GSO $\bbS_T= \bbV_T \bbLambda_T \bbV_T^{\herm}$ where $\bbV_T=[\bbv_{T,1},\dots,\bbv_{T,T}]$ is the matrix of temporal eigenvectors and $\bbLambda_T = \diag(\lambda_{T,1},\dots,\lambda_{T,T})$ is that of temporal eigenvalues. 
%where assuming temporal graph $\ccalG_T$ as a cyclic graph the eigenvectors $\bbV_T^\herm$ form the DFT matrix and the eigenvalues are $\bbLambda_T = \diag(  e^{-j2\pi 0/T},\dots,e^{-j2\pi (T-1)/T}	\big)$.
Then, the GSO of the product graph $\bbS_\diamond$ can be eigendecomposed as
%
\begin{equation}
\bbS_\diamond= \bbV_\diamond \bbLambda_\diamond\bbV_\diamond^\herm
= (\bbV_T \otimes \bbV)(\boldsymbol{\Lambda}_T \diamond \boldsymbol{\Lambda})(\bbV_T \otimes \bbV)^{\herm}
\end{equation}
%
with eigenvectors are $\bbV_\diamond=\bbV_T \otimes \bbV$ and eigenvalues $\bbLambda_\diamond = \boldsymbol{\Lambda}_T \diamond \boldsymbol{\Lambda}$ dictated by the product graph.
Then, we can define the graph-time Fourier transform of signal $\bbx_\diamond$ as $\tilde{\bbx}_{\diamond} =  (\bbV_T \otimes \bbV)^\herm \bbx_\diamond $~\cite{grassi2017time,sandryhaila2014big}.
This transform represents the variation of the multivariate time-series over the product graph in terms of product graph eigenvectors.
Using these concepts, the following proposition characterizes the spectral behavior of filter~\eqref{eq:graphtimegeneralfilter}.

%%%%%%%%%%%%%%%%%%
%	PROPOSITION
\begin{proposition}
	\label{prop3}
	Consider the eigendecomposition of the spatial GSO $\bbS = \bbV\bbLambda\bbV^\herm$ and the temporal GSO $\bbS_T = \bbV_T\bbLambda_T\bbV_T^\herm$.
	Consider also the graph-time Fourier transform of the output signal $\tilde{\bby}_\diamond = (\bbV_T \otimes \bbV)^\herm \bby_{\diamond}$ and the input signal  $\tilde{\bbx}_\diamond = (\bbV_T \otimes \bbV)^\herm \bbx_{\diamond}$.
	Then, the filtering operation~\eqref{eq:graphtimegeneralfilter} operates in the graph-time frequency domain as
	\begin{equation}
		\tilde{\bby}_{\diamond}= h\left(\boldsymbol{\Lambda}_T, \boldsymbol{\Lambda}\right) \tilde{\bbx}_\diamond
	\end{equation}
	with the filter frequency response matrix
	\begin{equation}
		h\left(\boldsymbol{\Lambda}_T, \boldsymbol{\Lambda}\right)
		= \sum_{k=0}^{\bar{K}} \sum_{l=0}^{\tilde{K}}h_{kl}(\bbLambda_T^l \otimes \bbLambda^k)
		\label{eq:spectral}
	\end{equation}
	with diagonal entries  $\left[h\left(\boldsymbol{\Lambda}_T, \boldsymbol{\Lambda}\right)\right]_{k k}=h\left( \lambda_{Tt}, \lambda_{i}\right)$ and $k=N(t-1)+i$ for $i=1, \ldots, N$ and $t=1, \ldots, T$.
\end{proposition}
\begin{proof}
	See Appendix.~\ref{sec:spectral}.
\end{proof}

That is, the graph-time filtered version $\bby_{\diamond}$ of $\bbx_{\diamond}$ with the filter $\bbH(\bbS_T,\bbS)$ corresponds to an element-wise multiplication in the graph-time frequency representation, i.e., $\hat{\bby}_{ti} = h([\bbLambda_T]_t,[\bbLambda]_i)\hat{\bbx}_{ti}$.
This is a direct extension of the convolution theorem~\cite{oppenheim1999discrete} to the spatiotemporal setting, ultimately, justifying the qualifier convolution for filter~\eqref{eq:graphtimegeneralfilter}. It shows that by learning the parameters ${h_{kl}}$ we not only learn spatiotemporal coupling in the vertex domain with desirable properties but also the frequency response of these filters to extract relevant spectral patterns.

%\red{EI: This is your former proposition. I did not touch it since you need to learn how to write them better. A proposition should be in this form: Given this and that. Then it follows that. Here: i) no need to assume unitary, we made that implicit above and it is not a relevant assumption for the proposition, you need to give the spatial GSO and temporal GSO with their eigendecompositions, then give the main equation only in the frequency domain in all variables not some in frequency some in the vertes; also first define index k and then give the k-th element of the matrix.}
%


%====================================================================================================================================================================================%
%====================================================================================================================================================================================%
%====================================================================================================================================================================================%
%
%\subsection{Spectral Analysis and permutation Equivariance}
%
%We can characterize the filter frequency response with respect to the product graph decomposition. Here, we exploit the eigendecomposition of $\bbS_\diamond$ considering the shift operator $\bbS= \bbV \bbLambda \bbV^{*}$ and $\bbS_T= \bbV_T \bbLambda_T \bbV_T^{*}$. Recall that $\bbV_T^*$ is the complex conjugate of the discrete Fourier transform (DFT) matrix and $\bbLambda_T$ is the diagonal matrix containing the eigenvalues $[\bbLambda_T]_{tt}= e^{-j2\pi (t-1)/T}$ with $j= \sqrt{-1}$ and $t=1, \ldots, T$ if the temporal graph be a line graph.
%
%Because the product-graph shift operator $\bbS_\diamond=\bbS_T \diamond \bbS$ is the linear combination of Kronecker product(s), we can eigendecompose it by exploiting the Kronecker product properties
%
%\begin{equation}
%\bbS_\diamond= \bbV_\diamond \bbLambda_\diamond\bbV_\diamond^*
%= (\bbV_T \otimes \bbV)(\boldsymbol{\Lambda}_T \diamond \boldsymbol{\Lambda})(\bbV_T \otimes \bbV)^{H}
%\end{equation}
%where $\bbV_\diamond=\bbV_T \otimes \bbV$ is the GFT basis of the product graph shift operator and the GFT coefficients cab be calculated by $\tilde{\bbx_{\diamond}} =  (\bbV_T \otimes \bbV)^H \bbx_\diamond $~\cite{grassi2017time}.% and it is also known as joint time-vertex Fourier transform (JFT)~\cite{grassi2017time}.
%Hence, we can define the graph-time Fourier decomposition for a signal $\bbx_\diamond$ over the product graph
%\begin{equation}
%	\bbx_\diamond =  (\bbV_T \otimes \bbV)\tilde{\bbx_{\diamond}} = \sum_{t=1}^{T}\sum_{i=1}^{N} \tilde{\bbx}_{ti} (\bbv_{Tt}\otimes\bbv_i)
%\end{equation}
%which indicates the signal variations on both time and space.
%
%\begin{proposition}
%	Assume $\bbV_\diamond$ is a unitary matrix, then operations such as filtering can be performed in the graph-time frequency domain, similar to the graph filters. In particular, the graph-time filtered version $\bby_{\diamond}$ of $\bbx_{\diamond}$ with the filter $\bbH(\bbS_T,\bbS)$ corresponds again to an element-wise multiplication, this time in the graph-time frequency representation, i.e., $\hat{\bby}_{ti} = h([\bbLambda_T]_t,[\bbLambda]_i)\hat{\bbx}_{ti}$, hence
%	\begin{equation}
%	\bby_{\diamond}=\bbH\left(\bbS_T,\bbS\right) \bbx_{\diamond} \triangleq \bbV_\diamond h\left(\boldsymbol{\Lambda}_T, \boldsymbol{\Lambda}\right) \bbV_\diamond^{*} \bbx_\diamond
%	\end{equation}
%	where $h\left(\boldsymbol{\Lambda}_T, \boldsymbol{\Lambda}\right)$ is the graph-time frequency response of the filter, with entries  $\left[h\left(\boldsymbol{\Lambda}_T, \boldsymbol{\Lambda}\right)\right]_{k k}=h\left( e^{-j2\pi (t-1)/T}, \lambda_{i}\right)$ and $k=N(t-1)+i$ for $i=1, \ldots, N$ and $t=1, \ldots, T$.
%\end{proposition}
%\begin{proof}
%	See Appendix. ?.
%\end{proof}

%An important property of graph-time filters is permutation equivariance which allows us to assign any arbitrary ordering to the nodes. This property can be stated formally as
%\begin{proposition}
%	Let $\bbx_\diamond = \text{vec}(\bbX)$ be a signal over product graph $\ccalG_\diamond$ with shift operator $\bbS_\diamond = \bbS_T \diamond \bbS$. Consider also the output of a graph-time filter $\bbH(\bbS_T,\bbS)\bbx_{\diamond}$. Then, for a permutation matrix $\bbP$, it holds that
%	\begin{equation}
%		\bbP^\top\text{vec}^{-1}(\bbH(\bbS_T,\bbS)\bbx_{\diamond}) = \bbH(\bbS_T,\bbP^\top\bbS\bbP)\text{vec}(\bbP^\top\bbX).
%	\end{equation}
%	This means the graph-time filter operating on a multivariate time-series is a permuted version of the graph-time filter operating on permuted spatial graph $\bbP^\top\bbS\bbP$.
%	So, if we permute the labeling of nodes, the output permutes in a similar manner.
%\end{proposition}
%\begin{proof}
%	See Appendix. ?.
%\end{proof}

%All of these spectral analysis and properties of graph-time filters allows us to have a better understanding of GTCNNs and enable us to investigate the limitations of the model. As an example, we apply these properties to prove the stability aspects of GTCNNs. 

==> GTCNN paper/Sections/Intro.tex <==

%% Motivation

Learning from \emph{multivariate temporal} data is a challenging task due to their intrinsic spatiotemporal dependencies.
This problem arises in applications such as time series forecasting, classification, action recognition, and anomaly detection~\cite{mo:yu2017spatio,mo:yan2018STGCNN,mo:kadous2002temporal,mo:zhang2019anomaly}.
The spatial dependencies can be captured by a graph either explicitly such as in transportation networks or implicitly such as in recommender systems~\cite{wang2021graph}.
Therefore, graph-based inductive biases should be considered during learning to exploit the spatial dependencies alongside with temporal patterns in a computationally and data efficient manner.
Based on advances in processing and learning over graphs~\cite{GSPsurvey,hamilton2017representation}, a handful of approaches have been proposed to learn from multivariate temporal data~\cite{surveyDLonST}.
The main challenge is to capture the spatiotemporal dependencies by built-in effective biases in a principled manner~\cite{battaglia2018inductivebias}.

% Convolution principle
The convolution principle has been key to build learning solutions for graph-based data \cite{gama2020elvinmagazine,bronstein2021geometric}. By cascading graph convolutional filters and pointwise nonlinearities, graph convolutional neural networks (GCNNs) have been developed as non-linear models for graph-based data~\cite{GamaGCNN,CNNonGraphs}. Such a principle reduces both the number of learnable parameters and the computational complexity in the GCNN, ultimately, overcoming the curse of dimensionality~\cite{battaglia2018inductivebias,bronstein2021geometric}. The convolution operation allows also for a mathematical tractability of GCNNs. On the one hand, it is a permutation equivariant operation, implying that it can capture structural symmetries to aid learning~\cite{Ruiz2021GNN,bronstein2021geometric}. On the other hand, it enjoys a spectral duality by means of a graph signal processing analysis \cite{GSPsurvey}, which, in turn, can be used to characterize the stability of GCNNs to perturbations in the support \cite{gamamain,gao2021stability,Ruiz2021GNN,levie2021transferability}. The overreaching goal of this paper is to leverage the convolution principle to learn from spatiotemporal data as well as study the theoretical properties of this model.

%% GCNN overview
%Graph convolutional neural networks (GCNNs) are powerful tools to process network data since they are non-linear models that account for the graph structure~\cite{gama2020elvinmagazine}.
%GCNNs are cascaded architectures of linear transformations and point-wise nonlinearities, but the transformation is substituted with a graph filter in each layer~\cite{GamaGCNN,GCN_Welling,CNNonGraphs}.
%GCNNs are cascaded architectures of graph convolutional filters and point-wise nonlinearities~\cite{GamaGCNN,GCN_Welling,CNNonGraphs}.
%Hence, GCNNs are equipped with the graph structure in a convolutional manner to exploit spatial dependencies for learning from non-Euclidean data~\cite{GeoDL}.
%The designed convolution principle in graph filters reduces the number of parameters in a GCNN rather than conventional graph neural networks.
%GCNNs also inherit two main properties of graph convolutional filters, namely, permutation equivariance and stability to perturbations in the support~\cite{gamamain,gao2021stability}.
%Permutation equivariance implies that the model captures structural symmetries in the graph, which enables GCNNs to exploit internal symmetries and aid learning~\cite{Ruiz2021GNN}.
%Stability states that small changes in the graph cannot affect the output considerably, so, GCNNs are transferable across slightly different graphs.
%We aim to follow a similar approach in a spatiotemporal manner and design a graph-time convolutional filter to benefit from convolution merits. 

%%%%%
% Subsection
\subsection{Related Works}\label{subsec:relW}

There are two stream of works related to this paper: one developing architectures; and one studying their stability.

\smallskip
\noindent\textbf{Architectures.} Spatiotemporal graph-based learning models can be divided into hybrid and fused models.
%
\emph{Hybrid} models combine distinct learning algorithms for graph and temporal data.
They use GCNNs to extract higher-level spatial features and process these features by a temporal RNN, CNN, or variants of them.
The works in~\cite{mo:chai2018bike,mo:manessi2020dynamic,mo:sun2020constructing} concatenate a GCNN by an LSTM where the former is applied per timestamp and the latter per node.
Instead, the work in~\cite{mo:khodayar2018spatio} uses an RNN followed by a GCNN.
Another work in~\cite{mo:yu2017spatio} uses a narrower graph convolutional layer in between two temporal gated convolution layers, whereas~\cite{wang2021behavioral} combines graph diffusion with temporal convolutions. 
Another approach is to ignore the graph structure and use temporal CNNs augmented by the attention mechanism to reduce the number of parameters and ease training~\cite{mo:guo2019attention}.
Graph WaveNet uses a gated dilated temporal convolution followed by a first order graph convolution~\cite{mo:wu2019graph}.
%The advantage of hybrid models lies within their simple and efficient implementation since they benefit from modular spatial and temporal blocks.
%However, this modularity makes it unclear how to best combine them for the task at hand and to analyze theoretically their inner-working mechanisms.
%
%
%the combination of these blocks is blurred for learning spatiotemporal relationships effectively.
%It is also challenging to analyze these models theoretically and derive any sort of guarantees about their inner-working mechanisms or performance.
%
%
\emph{Fused} models impose the graph structure into conventional spatiotemporal models to jointly capture the spatiotemporal relationships~\cite{mo:isufi2019VARMA,mo:seo2018GRNN,mo:ruiz2020gatedGRNN,mo:si2019AEGCLSTM,mo:yan2018STGCNN}.
The fully connected blocks are replaced by graph convolutions to generate graph-based latent embeddings.
The work in~\cite{mo:isufi2019VARMA} proposed graph-based VARMA to learn spatiotemporal embeddings.
The authors in~\cite{mo:seo2018GRNN,mo:si2019AEGCLSTM} employ variants of RNN models with graph convolution-based blocks, while \cite{mo:ruiz2020gatedGRNN} also designs a graph-based gating module.
In another approach, the spatial graph is passed through a continuous temporal shift operator to define a spatiotemporal convolution~\cite{hadou2021space}. 
The work in~\cite{mo:yan2018STGCNN} starts with a graph partitioning and defines a spatiotemporal neighborhood in each partition to perform message passing.
The works in~\cite{pareja2020evolvegcn,ehsan2019variational} use diffusion schemes where the output is a function of the signals of at most one hop neighbors. Since diffusion is considered in a causal fashion the information from the k-hop spatiotemporal neighbors is considered in subsequent layers, which may be limiting to extract patterns.

%\red{EI: does this not use the cartesian product graph? Shouldn't we say it and make clear how we differ from it? Also the ST-GNN should be included here. We can say that prior to them in [1] we proposed the use of the convolution and here we elaborate on it more in detail; but say also how our architecture differs from theirs. We can say the differences in the following paragraph, which I discuss both hybrid and fused.}
%\green{MS: I gave a bit deeper look and it is not the gcn variant of our method for cartesian pg, it is first order filter of recursive model for cartesian.}
%Fused models can exploit spatiotemporal patterns due to their intrinsic graph-time dependent structure.
%However, these models mostly use low-order spatiotemporal aggregation which declines their efficiency in capturing spatiotemporal patterns.
%\blue{We address this challenge by leveraging product graphs}

%% comparison nd gaps
The advantage of hybrid models lies within their simple and efficient implementation since they benefit from modular spatial and temporal blocks.
However, this modularity makes it unclear how to best combine them for the task at hand and analyze theoretically their inner-working mechanisms.
Moreover, they are disjoint and sequential in nature (first graph and then temporal processing or vice-versa); thus, are more restrictive and require each node to accumulate global information.
Instead, fused models overcome these issues but they mostly use a low-order spatiotemporal aggregation which limits their effectiveness in capturing spatiotemporal patterns.
We address this challenge by leveraging product graphs to represent multivariate time series~\cite{sandryhaila2014big}.
Product graphs have been widely used for modeling complex data~\cite{leskovec2010kronecker}, the matrices~\cite{huang2018rating}, and developing a graph-time signal processing framework \cite{grassi2017time}.
However, their use for learning from spatiotemporal data has been limited.
The work in~\cite{pan2020spatio} builds spatiotemporal scattering transforms using product graphs and shows their advantages over alternative data representative solutions.
Here, we use product graphs as a platform to run spatiotemporal convolutions and build neural network solutions with it.
The work in \cite{mo:yan2018STGCNN} implicitly uses the Cartesian product graph to build a spatiotemporal neighborhood.
Differently, we develop a principled convolutional framework for learning via any product graph, multi-resolution neighborhood information aggregation in each layer (~\cite{mo:yan2018STGCNN} focuses only on immediate neighbors), and introduce a parametric product graph to learn the spatiotemporal coupling.



%\blue{
%One effective way to capture spatiotemporal patterns is to consider time as a graph;
%so, the time-varying signal converts into a static signal over this graph~\cite{sandryhaila2013discrete};
%and the spatiotemporal data can be seen as a time-invariant signal over the product graph between the spatial and the temporal graph~\cite{sandryhaila2014big}.
%This approach has proved its effectiveness in different problems, such as graph-time Fourier transform~\cite{grassi2017time}, autoregressive models~\cite{isufi2016armagraph,romero2071kernelbased}, and signal interpolation~\cite{lecun1995convolutional}.}
%\red{EI: this was before in the stability part. See what you can take from it and embed in the paragraph above.}



\smallskip
\noindent\textbf{Stability.}
Studying the stability of graph neural networks to graph perturbation reveals their potentials and limitations w.r.t. the underlying support.
The work in~\cite{gamamain} provided a stability scheme to relative perturbations on the graph for GCNNs by enforcing graph convolutional filters to vary smoothly over high graph frequencies.
Authors in~\cite{levie2019transferability} proposed a linear stability bound to graph arbitrary perturbation for a large class of graph filters named Cayley smooth space.
The work in~\cite{thanou2021stability} considers an edge rewiring model for perturbation and provides an upper bound for output changes.
The authors in~\cite{gao2021stability} proved that GCNNs are stable to stochastic perturbation model where links have a probability of existence in the graph.
In case of spatiotemporal graph neural networks, the work in~\cite{mo:ruiz2020gatedGRNN} developed a stability analysis to graph perturbation following the model in~\cite{gamamain}.
The authors in~\cite{hadou2021space} have used the relative perturbation model in~\cite{gamamain} to investigate their model stability properties. 
We also pursue a similar analysis as~\cite{gamamain} for the graph-time convolutional neural network to approve its capabilities and observe the effects of time component in the stability and transferability  properties of them.
The similar base of stability analysis allows us to compare the proposed model with previous works in~\cite{mo:ruiz2020gatedGRNN,hadou2021space} and collect insights into how different learning solutions for spatiotemporal data handle uncertainty in the spatial support.
Differently from the latter, the proposed stability results via product graphs provides direct links with that of GCNNs if time is invariant, highlighting also the impact of how the temporal component is accounted for a joint spatiotemporal learning.
%% Gaps
%The advantage of hybrid models lies within their simple and efficient implementation since they benefit from modular spatial and temporal blocks.
%However, the combination of these blocks is blurred for learning spatiotemporal relationships effectively.
%It is also challenging to analyze these models theoretically and derive any sort of guarantees about their inner-working mechanisms or performance.
%On the other hand, these spatiotemporal patterns can be exploited by fused models due to their intrinsic graph-time dependent structure.
%One effective way to capture spatiotemporal patterns is to consider time as a graph;
%so, the time-varying signal converts into a static signal over this graph~\cite{sandryhaila2013discrete};
%and the spatiotemporal data can be seen as a time-invariant signal over the product graph between the spatial and the temporal graph~\cite{sandryhaila2014big}.
%This approach has proved its effectiveness in different problems, such as graph-time Fourier transform~\cite{grassi2017time}, autoregressive models~\cite{isufi2016armagraph,romero2071kernelbased}, and signal interpolation~\cite{lecun1995convolutional}.

%%%%%
% Subsection
\subsection{Contribution}\label{subsec:contrib}

We consider the convolutional principle over product graphs as an inductive bias to build graph-time convolutional neural network (GTCNN) for learning from multivariate temporal data. Our specific contributions are:

% Contribution
%In this paper, we propose a graph-time convolutional neural network (GTCNN) where each layer performs a graph-time convolution over product graphs.
%Furthermore, we prove permutation equivariance and stability properties of GTCNNs to expose their strength in learning from multivariate temporal data.
%Our contribution is threefold:
\begin{enumerate}[label=C\arabic*)]
	\item \emph{Principled architecture:} We develop an architecture that leverages graph-time convolutions and product graphs as a spatiotemporal inductive bias to reduce the computational cost and the number of trainable parameters.
	% to the order of the graph sparsity and an order one number of trainable parameters.
	We also propose a solution to learn the spatiotemporal coupling and a recursive implementation to tackle the high dimensionality of the product graphs.
%	\item
%	We generalize the GTCNN into a parametric product graph GTCNN that learns also the spatiotemporal coupling in an efficient way, which means the dependency among nodes through time is leveraged in an end-to-end learning problem. For this more general form we show it is permutation equivariant and analyze the spectral response by means of a graph-time Fourier transform.
	\item \emph{Theoretical properties:}
	%The convolution principle jointly over graph and time allows for a theoretical analysis of the layers. 
	We prove GTCNNs are permutation equivariant. Then, leveraging concepts from graph-time signal processing, we show the learned filters act in the joint graph and temporal spectral domain as point-wise multiplication between the learnt frequency response and the graph-time Fourier transform of the input.
	%
	%we leverage concepts from joint graph-time signal processing to show that in the spectral domain the learned filters act as a point-wise multiplication between the learnt frequency response and the graph-time Fourier transform of the input.
	\item \emph{Stability:}
	%Leveraging the convolution principle and its spectral equivalent, 
	We prove the GTCNN is stable to perturbations in the spatial graph. Our result shows the GTCNN becomes less stable for larger graphs and that the temporal window in the product graph affects it more severely than increasing the number of nodes. We provide a thorough discussion of our stability bound w.r.t. baselines and alternative approaches.
%	how time component contributes in the stability properties of the GTCNN. The solution generally become less stable for larger graphs and we have shown time can affect it more severely than the number of nodes. This result contributes to the recent advances about the stability of GNNs.
	\item  \emph{Numerical performance:} We compare the GTCNN with baseline and state-of-the-art solutions in different tasks about time series classification and forecasting. The GTCNN outperforms the baseline GCNN model that ignores the temporal dimension and compares well with alternatives on benchmark datasets.
%	The GTCNN performs better than a baseline GCNN and allowing the model to learn spatiotemporal coupling increases the performance. They also compare well with state-of-the-art and baselines on benchmark datasets such as traffic PEMS-Bay and METR-LA, and weather datasets Molene and NOAA.
\end{enumerate}


%% Structure
The structure of this paper is as follows.
In Section.~\ref{sec_back}, we explain product graphs and signals over them to formulate our problem.
In Section.~\ref{sec_gtcnn}, the GTCNN is proposed and its properties are discussed.
Section.~\ref{sec_stability} is dedicated to stability analysis of GTCNNs.
Section.~\ref{sec_numeric} contains the numerical results and experiments to corroborate the strengths of GTCNNs.
Finally, Section~\ref{sec_conc} concludes the paper.


%\red{EI: we have three contributions. i) We develop a principled GTCNN architecture based on the convolution and product graphs, which is local and efficient; ii) We generalize the GTCNN into a parametric PG-GTCNN that learns also the spatiotemporal coupling in an efficient way etc etc.. For this more general form we show it is permutation equivariant and analyze the spectral response by means of a graph-time Fourier transform; ii) We prove GTCNNs are stable to perturbation under Lipsitz properties on the filter in the graph, which extends the findings of Gama to a more general case, where the latter do not hold.}

==> GTCNN paper/Sections/Numerical.tex <==
This section evaluates the GTCNN performance in different scenarios and compares it with other state-of-the-art algorithms. In all experiments, the ADAM optimizer is used to train the model and an unweighted directed line graph is selected as the temporal graph.

\subsection{Source Localization}
The task is to detect the source of a diffusion process over a graph by observing the time-series of length $T$.
The graph is an undirected stochastic block model with $C = 5$ communities and $N = 100$ nodes.
The edges are randomly and independently drawn with probability $0.8$ for nodes in a same community and $0.2$ for nodes in different communities.
At $t=0$, a random node takes a unitary value and diffuses it throughout the network 30 times as $e^{-t\bbL}$.
The model is fed with a multivariate time series $\{\bbx_{t-T},\dots,\bbx_{t-1}\}$ randomly selected after at least $t = 15$ diffusion and the goal is to detect the community corresponding to the source node.  
Our aim here is to study the role of the different product graphs; hence, we compare different GTCNNs with the baseline GCNN that ignores the temporal connections and treats time as feature.

%To accent the role of GTCNN and its stability properties, we designed a synthetic experiment for this task allowing us to control problem parameters and have access to the ground-truth graph.

The dataset contains $2000$ samples with an $80/10/10$ split.
%Each sample is a diffused signal over the graph with a source belonging to a random community.
All architectures have two layers with two second order filters.
The cross-entropy loss is used for all models except for the parametric which its cost is also regularized by an $l_1$-norm of product graph parameters $\{s_{ij}\}$ with regularization weight $\beta = 0.05$ to enforce sparse spatiotemporal connections.
The temporal windows are selected from $T\in\{2,3,4,5\}$ and the features from $F_1,F_2\in\{4,8,16,32\}$.
%Hence, the task is a classification problem which assigns a community to the multivariate time-series .
%To compare GTCNN with the baseline GCNN, we considered $T$ consecutive graph signals as distinct features.
The models are trained for $1000$ epochs with $100$ batch size.
Each experiment is done for $10$ different random graphs and $10$ different dataset realization.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{Figures/exp1.png}
	\caption{Comparison of GCNN with parametric and non-parametric GTCNN performances on source localization task to emphasize on the role of spatiotemporal couplings.}
	\label{fig:exp1}
\end{figure}

The results in Fig.~\ref{fig:exp1} suggest that accounting for the temporal connections even through a fixed product graph improves the performance.
Considering consecutive times as features in the GCNN can be translated as a fully connected temporal graph, so, the improved performance by enforcing a reasonable structure to temporal samples was expected.  
Better results are achieved by using parametric product graph as it learns the temporal connections for the specific task.
This flexibility reduces also the number of failed training attempts compared with the fixed product graphs and the GCNN.
%However, the downside of parametric and recursive models are their higher variance in the results.



\subsection{Multivariate Time-Series Forecasting}

\begin{table*}[t]
	\centering
	\caption{Performance comparison of GTCNN and other baseline models for different prediction horizons. The best performance is shown in bold and the second best is underlined.
	  The standard deviation of all models are of the order $10^{-3}$ and are omitted to avoid an overcrowded table.}
	\label{tablemain}
	\renewcommand{\arraystretch}{1.5}
	\begin{tabular}{|ll|lll|lll|lll|}
		\hline
		\multirow{2}{*}{Data}     & \multirow{2}{*}{Models} & \multicolumn{3}{c|}{3-Steps}                    & \multicolumn{3}{c|}{6-Steps}                    & \multicolumn{3}{c|}{12-Steps}                    \\ \cline{3-11} 
		&                         & MAE           & RMSE          & MAPE            & MAE           & RMSE          & MAPE            & MAE           & RMSE          & MAPE             \\ \hline
		\multirow{8}{*}{\begin{sideways}METR-LA\end{sideways}}
		& ARIMA~\cite{li2017diffusion}                   
		& 3.99          & 8.21          & 9.60\%          & 5.15          & 10.45         & 12.70\%         & 6.90          & 13.23         & 17.40\%          \\
		& G-VARMA~\cite{mo:isufi2019VARMA}                 
		& 3.60          & 6.89          & 9.62\%          & 4.05          & 7.84          & 11.22\%         & 5.12          & 9.58          & 14.00\%          \\
		& GP-VAR~\cite{mo:isufi2019VARMA}                  
		& 3.56          & 6.54          & 9.55\%          & 3.98          & 7.56          & 11.02\%         & 4.87          & 9.19          & 13.34\%          \\
		& FC-LSTM~\cite{li2017diffusion}                  & 3.44          & 6.30          & 9.60\%          & 3.77          & 7.23          & 10.90\%         & 4.37          & 8.69          & 13.20\%          \\
		& Graph Wavenet~\cite{mo:wu2019graph}           
		& \ul{2.69}     & \textbf{5.15} & \ul{6.90\%}     & \ul{3.07}     & \ul{6.22}     & \ul{8.37\%}     & \textbf{3.53} & \ul{7.37}     & \textbf{10.01\%} \\
		& STGCN~\cite{mo:yu2017spatio}                   
		& 2.88          & 5.74          & 7.62\%          & 3.47          & 7.24          & 9.57\%          & 4.59          & 9.40          & 12.70\%          \\
		& GGRNN~\cite{mo:ruiz2020gatedGRNN}                  
		& 2.73          & 5.44          & 7.12\%          & 3.31          & 6.63          & 8.97\%          & 3.88          & 8.14          & 10.59\%          \\
		& GTCNN (this work)                   & \textbf{2.68} & \ul{5.17}     & \textbf{6.85\%} & \textbf{3.02} & \textbf{6.20} & \textbf{8.30\%} & \ul{3.55}     & \textbf{7.35} & \ul{10.21\%}          \\ \hline
		\multirow{8}{*}{\begin{sideways}PEMS-BAY\end{sideways}}
		& ARIMA~\cite{li2017diffusion}                  
		& 1.62          & 3.30          & 3.50\%          & 2.33          & 4.76          & 5.40\%          & 3.38          & 6.50          & 8.30\%           \\
		& G-VARMA~\cite{mo:isufi2019VARMA}                 
		& 1.88          & 3.96          & 4.28\%          & 2.45          & 4.70          & 5.42\%          & 3.01          & 5.83          & 7.10\%           \\
		& GP-VAR~\cite{mo:isufi2019VARMA}                  
		& 1.74          & 3.22          & 3.45\%          & 2.16          & 4.41          & 5.15\%          & 2.48          & 5.04          & 6.18\%           \\
		& FC-LSTM~\cite{li2017diffusion}                   & 2.05          & 4.19          & 4.80\%          & 2.20          & 4.55          & 5.20\%          & 2.37          & 4.74          & 5.70\%           \\
		& Graph Wavenet~\cite{mo:wu2019graph}           
		& \ul{1.30}     & \ul{2.74}     & \ul{2.73\%}     & \textbf{1.63} & \ul{3.70}     & \textbf{3.67\%} & \textbf{1.95} & \textbf{4.52} & \textbf{4.63\%}  \\
		& STGCN~\cite{mo:yu2017spatio}                   
		& 1.36          & 2.96          & 2.90\%          & 1.81          & 4.27          & 4.17\%          & 2.49          & 5.69          & 5.79\%           \\
		& GGRNN~\cite{mo:ruiz2020gatedGRNN}                   
		& 1.33          & 2.81          & 2.83\%          & 1.68          & 3.94          & \ul{3.79\%}     & 2.34          & 5.14          & 5.21\%           \\
		& GTCNN (this work)                   & \textbf{1.25} & \textbf{2.66} & \textbf{2.61\%} & \ul{1.65}     & \textbf{3.68} & 3.82\%          & \ul{2.27}     & \ul{4.99}     & \ul{5.11\%}      \\ \hline
	\end{tabular}
	\renewcommand{\arraystretch}{1}	
\end{table*}

We applied the GTCNN to address traffic and weather forecasting on four benchmark datasets.
On the traffic forecasting task, we used parametric product graph while the recursive model is applied for the weather forecasting problem.
The goal is to show that both solutions compare well with alternatives.
The results are compared with baseline methods to provide insights into the GTCNN capabilities and limitations. 
For baselines, we considered:
\begin{itemize}
	\item \textit{ARIMA}:
	auto-regressive integrated moving average model using Kalman filter~\cite{li2017diffusion}. This model treats each time series individually.
	\item \textit{G-VARMA}:
	graph vector auto-regressive moving average model~\cite{mo:isufi2019VARMA}. This model works upon statistical assumptions on the data and takes the spatial graph into account.
	\item \textit{GP-VAR}:
	graph polynomial auto-regressive model~\cite{mo:isufi2019VARMA}. It has fewer parameters than G-VARMA yet considers the spatial graph.
	\item \textit{FC-LSTM}~\cite{li2017diffusion}:
	fully connected LSTM performing independently on time series, i.e., one LSTM per time series.
	\item \textit{Graph WaveNet}:
	A hybrid convolutional model for time-series over graph~\cite{mo:wu2019graph}.
	\item \textit{STGCN}:
	spatial-temporal graph convolution network which uses graph convolution module alongside with 1D convolution~\cite{mo:yu2017spatio}.
	\item \textit{GGRNN}:
	gated graph recurrent neural network which replace linear transforms in a RNN by graph convolutional filters~\cite{mo:ruiz2020gatedGRNN}.
\end{itemize}

\medskip \noindent
\textbf{Traffic forecasting.}
We considered the traffic network datasets METR-LA and PEMS-BAY.
METR-LA contains four months of recorded traffic data over 207 nodes on the highways of Los Angeles County with 5 minutes resolution~\cite{li2017diffusion}.
PEMS-BAY includes six months of traffic information over 325 nodes in Bay Area with similar resolution of METR-LA.
We considered the same setting as in~\cite{shuman2013emerging}.
The shift operator is a directed adjacency matrix constructed by applying a Gaussian threshold kernel over the road network distance matrix.
The goal is to predict the traffic load in time horizons $15-30-60$ minutes having the time series for last 30 minutes, i.e., $T = 6$.

Both datasets are divided into an $80/10/10$ split chronologically.
The GTCNN is fixed and contains two layers with third order filters and the parametric product graph.
We evaluated the number of features in each layer from $F \in \{4,8,16\}$.
The objective function is the regularized mean squared error (MSE) via the $l_1$-norm on the product graph parameters $\bbs$, i.e., $\ccalL = \text{MSE}(\hat{\bbx}_{t+1},\bbx_{t+1}) + \beta \|\bbs \|_1$.
The regularization weight is chosen from $\beta \in \{0,0.05,0.1\}$.
For the GGRNN, we evaluated features $F \in \{4,8,16\}$ and filter orders $K \in \{3,4,5\}$.
For the other models, the parameters have been set similar to~\cite{mo:wu2019graph}.
The evaluation metrics are the mean absolute error (MAE), the root mean squared error (RMSE), and the mean absolute percentage error (MAPE).

Table~\ref{tablemain} compares the performance of GTCNN and other baseline models.
The GTCNN outperforms the other models in a short horizon while Graph WaveNet works better for longer horizons.
The benefits in the short term are due to high order spatiotemporal aggregation in the GTCNN which allows capturing efficiently the spatiotemporal patterns in the data.
On the longer term, the Graph WaveNet works better because it captures longer term patterns by increasing the receptive field of the model through dilated convolutions.
Graph Wavenet can also be fed with a longer time series as it works only with the spatial graph. 
Differently, the GTCNN does not capture them and an efficient implementation remains an interesting extension.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

\medskip \noindent
\textbf{Weather forecasting.}
We considered two benchmark datasets, Molene and NOAA.
The Molene dataset contains 744 hourly temperature measurement across 32 stations in a region of France.
The NOAA dataset contains 8579 hourly temperature measurement across 109 stations in the U.S..
The same setting as~\cite{mo:isufi2019VARMA} is used in this experiment.
Our aim is to make a prediction of the temperature for $1-3-5$ hours ahead having the time series for last 10 hours.

The model is fixed and consists of two recursive GTCNN [c.f.~\eqref{eq:graphtimegeneralfilter}] layers with temporal locality selected from $\tilde{K} \in\{3,4,5\}$ and spatial locality from $\bar{K} \in \{3,5,7\}$.
For the neural network models, the number of features is chosen via grid search from $F\in\{4,8,16\}$.
The GGRNN filter orders are varied among $K \in \{3,4,5\}$.
For the statistical models we set the parameters similar to~\cite{mo:isufi2019VARMA}.
The number of LSTM hidden units are selected from $\{8,16,32,64\}$.
The loss function is the MSE at 1-step prediction.

Table~\ref{tableweather} indicates the model performance for different prediction horizons.
In the Molene dataset, graph-based statistical methods outperform the rest as the dataset contains fewer samples and the time series have clear patterns in their temporal variation.
Hence, leveraging a statistical assumption for the data compensates for the lack of samples and leads to a better performance.
Among these methods, G-VARMA performs the best which indicates the importance of inducing the graph in the model.
Due to the temporal connections, the GTCNN still performs better than the neural network counterparts.
In the NOAA dataset, the abundance of training data allows the neural network models to learn complicated patterns and outperform statistical-based models. All the neural network alternatives perform closely, however, in higher forecasting horizons LSTM starts to take over the other variants while GTCNN performs better in short horizons.
Overall, the GTCNN can be considered as a valid alternative for learning spatiotemporal representations in both cases where the training set is limited or large.




\begin{table*}[]
	\centering
	\caption{The performance of the GTCNN compared with baseline methods on the weather forecasting task. The best performance is shown in bold and the second best is underlined.
	The standard deviation of all models are of the order $10^{-2}$ for the Molene dataset and $10^{-3}$ for the NOAA dataset and they are omitted to avoid an overcrowded table.}
	\label{tableweather}
	\renewcommand{\arraystretch}{1.5}
%	\begin{tabular}{|l|lll|lll|}
%		\hline
%		\multirow{2}{*}{Models} & \multicolumn{3}{c|}{Moelene}                     & \multicolumn{3}{c|}{NOAA}                        \\ \cline{2-7} 
%		& 1-step         & 3-step         & 5-step         & 1-step         & 3-step         & 5-step         \\ \hline
%		ARIMA~\cite{li2017diffusion}                   & 0.225          & 0.394          & 0.581          & 0.047          & 0.174          & 0.314          \\
%		G-VARMA~\cite{mo:isufi2019VARMA}                 & \textbf{0.209} & \textbf{0.381} & \textbf{0.567} & 0.043          & 0.151          & 0.255          \\
%		GP-VAR~\cite{mo:isufi2019VARMA}                  & \ul{0.212}    & \ul{0.389}    & \ul{0.572}    & 0.049          & 0.152          & 0.281          \\
%		LSTM                    & 0.382          & 0.521          & 0.741          & 0.036          & \ul{0.072}    & \textbf{0.151} \\
%		Graph Wavenet~\cite{mo:wu2019graph}           & 0.351          & 0.496          & 0.712          & 0.040          & 0.103          & \ul{0.154}          \\
%		STGCN~\cite{mo:yu2017spatio}                   & 0.377          & 0.504          & 0.709          & 0.042          & 0.089          & 0.182          \\
%		GGRNN~\cite{mo:ruiz2020gatedGRNN}                   & 0.316          & 0.503          & 0.695          & \textbf{0.031} & 0.091          & 0.177          \\
%		GTCNN                   & 0.354          & 0.489          & 0.618          & \ul{0.034}    & \textbf{0.069} & 0.166    \\ \hline
%	\end{tabular}
	\input{Figures/table2}
	\renewcommand{\arraystretch}{1}
\end{table*}

\subsection{Stability Analysis}

\begin{figure*}
	\centering
	\begin{subfigure}[b]{0.22\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/exp2.png}
		\caption{}
		\label{fig:exp2}
	\end{subfigure}
	\hfill	
	\begin{subfigure}[b]{0.22\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/exp3.png}
		\caption{}
		\label{fig:exp3}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.22\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/exp5.png}
		\caption{}
		\label{fig:exp4}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.22\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/exp6.png}
		\caption{}
		\label{fig:exp5}
	\end{subfigure}\hfill
	\caption{
			 Stability results for different scenarios of the parametric GTCNN and the best alternative for a fixed product graph (Kronecker, Cartesian, Strong). We also consider the vanilla GCNN as a baseline.
			 (a) Results for different SNRs.
			 (b) Performance for different graph sizes in 5dB perturbation.
			 (c) Embedding difference in terms of rNMSE between the trained GTCNN on the nominal graph and the perturbed one.
			 (d) Embedding difference for different time series lengths in 5dB perturbation.
			}
	\label{fig:staball}
\end{figure*}

To investigate the stability of the GTCNN, we tested the trained models in the source localization experiment under perturbed graphs with different signal to noise ratios (SNR)
\begin{equation}
	\textnormal{SNR} = 10\log_{10} \frac{\|\bbS\|^2_F}{2\|\bbE\|_F^2}.
\end{equation}
The noise energy is doubled as it appears twice in the relative perturbation model [c.f.~\eqref{relperturb}].

Fig.~\ref{fig:exp2} shows the average classification accuracy for different amounts of perturbations.
The GTCNN performs decently even in noisy scenarios around $5dB$.
Fig.~\ref{fig:exp3} represents the performance for different number of nodes in the graph.
We trained the GTCNN over different graph sizes and evaluated the results using a perturbed graph to observe the effect of graph size on stability.
The accuracy reduces steadily with the graph size as Theorem~\ref{filterstanility} suggests.
%The parametric product graph failed to be trained as it requires massive amount of memory while recursive version run smoothly thanks to the recursive implementation.

To investigate GTCNN stability itself and its relation with bound~\eqref{stabilitybound}, we analyzed the output embeddings of a fixed GTCNN network between the nominal and the perturbed graph.
Fig.~\ref{fig:exp4} and~\ref{fig:exp5} depicts theoretical bound versus GTCNN empirical performance.
We can observe that the bound reflects the same behavior of the empirical results with respect to both noise energy and time series length.
In addition, from all results we see the GTCNN offers a more stable performance compared with the vanilla GCNN by using the temporal data as features. This in turn highlights our theoretical insights after Theorem~\ref{filterstanility}.

Finally, in Fig.~\ref{fig:ffrfr} we investigate the frequency response of the learned filters.	
%Fig.~\ref{fig:ffrfr} illustrates the normalized frequency response of a trained recursive GTCNN on source localization task.
The frequency responses vary smoothly over high graph frequencies for the trained filters while the temporal frequencies have more variations throughout of the spectrum.
%Hence, there is no guarantee for the GTCNN to be stable after training phase unless its constraint forced in the loss function.


\begin{figure*}
		\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/filterResponse.png}
		\caption{}
		\label{fig:ffr}
	\end{subfigure}
	\hfill	
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/filterResponse2.png}
		\caption{}
		\label{fig:ffr2}
	\end{subfigure}
	\hfill
	\caption{ (a)~Normalized frequency response of a trained recursive GTCNN with two layers and four filters per layer. The bright color represents 1 while the dark color stands for 0.
	(b)~Examples of the filter frequency response variation to normalized frequencies.
	continuous line belongs to graph frequencies $\lambda$ and dashed ones are related to temporal frequencies $\lambda_T$. }	
\label{fig:ffrfr}
\end{figure*}

==> GTCNN paper/Sections/PermEqui_proof.tex <==
Let $\ccalG$ and its permuted version $\ccalG^\prime$ be represented by the GSOs $\bbS$ and $\bbS^\prime = \bbP^\top\bbS\bbP$, respectively, and let $\bbX^\prime = \bbP^\top\bbX$ be the spatial-graph permuted version of $\bbX$.
Considering the graph-time convolutional filter in~\eqref{eq:graphtimegeneralfilter}, the output for permuted signal and spatial graph is
\begin{equation}
	\bby_\diamond^\prime=
	\sum_{k=0}^{\bar{K}}
	\sum_{l=0}^{\tilde{K}}
	h_{kl} (\bbS_T^l \otimes (\bbP^\top\bbS\bbP)^k)\text{vec}(\bbP^\top\bbX)
	\label{eq:permeq_1}
\end{equation}
Invoking properties of permutation matrix $\bbP^k = \bbP$ and $\bbP^\top\bbP = \bbI_N$, the permuted spatial shift can be written as $(\bbP^\top\bbS\bbP)^k = \bbP^\top\bbS^k\bbP $.
Applying the mixed-product property for Kronecker product, we can rewrite~\eqref{eq:permeq_1} as
\begin{align}
	\bby_\diamond^\prime &=
	\sum_{k=0}^{\bar{K}}
	\sum_{l=0}^{\tilde{K}}
	h_{kl} (\bbI_T\bbS_T^l\bbI_T \otimes \bbP^\top\bbS^k\bbP)\text{vec}(\bbP^\top\bbX) \nonumber \\
	&= (\bbI_T\otimes\bbP^\top)\sum_{k=0}^{\bar{K}}
	\sum_{l=0}^{\tilde{K}}h_{kl} (\bbS_T^l \otimes \bbS^k)
	(\bbI_T\otimes\bbP)\text{vec}(\bbP^\top\bbX) \nonumber \\
	&=(\bbI_T\otimes\bbP^\top)\bbH(\bbS_T,\bbS)(\bbI_T\otimes\bbP)\text{vec}(\bbP^\top\bbX).
	\label{eq:permeq_2}
\end{align}
Now, we employ vector operator property $\text{vec}(\bbA\bbX\bbB)= (\bbB^\top \otimes \bbA)\text{vec}(\bbX)$ followed by the fact that permutation matrix is unitary $\bbP^\top\bbP = \bbI_N$ to write
\begin{equation}
	(\bbI_T\otimes\bbP)\text{vec}(\bbP^\top\bbX) = \text{vec}(\bbP\bbP^\top\bbX)
	=\text{vec}(\bbX).
	\label{tmp22}
\end{equation}
By replacing~\eqref{tmp22} into~\eqref{eq:permeq_2}, we have
\begin{align}
	\bby_\diamond^\prime
	&= (\bbI_T\otimes\bbP^\top)\bbH(\bbS_T,\bbS)\text{vec}(\bbX) \nonumber \\ 
	&=
	(\bbI_T\otimes\bbP^\top)\text{vec}(\bbY).
	\label{tmp23}
\end{align}
Expression~\eqref{tmp23} alongside with the vector operator property leads to
\begin{equation}
	\bby_\diamond^\prime=
	\text{vec}(\bbP^\top\bbY)
%	\text{vec}(\bbP^\top\text{vec}^{-1}(\bbH(\bbS_T,\bbS)\bbx_{\diamond}))
	\label{eq:permeq_3}
\end{equation}
Hence, $\bbY^\prime = \bbP^\top\bbY$ and the output is permuted similarly as the input.
Combining the results from~\eqref{eq:permeq_1} and~\eqref{eq:permeq_3} shows that the graph-time convolutional filter in~\eqref{eq:graphtimegeneralfilter} is permutation equivariant, i.e.,
\begin{equation}
		\text{vec}(\bbP^\top\text{vec}^{-1}(\bbH(\bbS_T,\bbS)\bbx_{\diamond})) = \bbH(\bbS_T,\bbP^\top\bbS\bbP)\text{vec}(\bbP^\top\bbX).
\end{equation}

Since GTCNNs are a composition of graph-time convolutional networks and point-wise nonlinearities, they also benefit from permutation equivariancy.
%
%\begin{align}
%	\bbP^\top\text{vec}^{-1}(&\Phi(\bbx_\diamond;\ccalH(\bbS_T,\bbS))) = \nonumber \\ &\Phi(\bbx_\diamond;\ccalH(\bbS_T,\bbP^\top\bbS\bbP))\text{vec}(\bbP^\top\bbX).
%\end{align}


==> GTCNN paper/Sections/Proof.tex <==
\begin{theorem}
	Let $\bbS = \bbV\Lambda\bbV^H$ and $\bbS_T\bbV_T\Lambda_T\bbV_T^H$ be spatial and temporal graph shift operators respectively.
	Assume $\hat{\bbS}$ is the relatively perturbed graph shift operator, i.e., $\bbP^\top\hat{\bbS}\bbP = \bbS + (\bbE\bbS + \bbS\bbE)$ where $\bbP$ is a permutation matrix and $\bbE = \bbU \bbM \bbU^H \in \ccalE(\bbS,\hat{\bbS})$ is the error matrix with a bounded norm
	\begin{equation}
		d(\bbS,\hat{\bbS}) \leq \|\bbE\|\leq \eps.
		\label{errorbound}
	\end{equation}
	For an integral Lipschitz spatial-temporal graph filter with respect to spatial eigenvalues
	\begin{equation}
		\lambda \frac{\partial h(\lambda_T,\lambda)}{\partial \lambda} \leq C
		\label{lipsch}
	\end{equation}
	the operator distance modulo permutation between filters $\bbH(\bbS_T,\bbS)$ and $\bbH(\bbS_T,\hat{\bbS})$ satisfies
	\begin{equation}
		\|\bbH(\bbS_T,\bbS) - \bbH(\bbS_T,\hat{\bbS}) \|_\ccalP \leq 2C\eps(1+T\delta \sqrt{NT}) + \ccalO(\eps^2)
	\end{equation}
	where $\delta = (\|\bbU-\bbV\|_2 +1)^2-1$ indicates the eigenvector misalignment between the spatial graph shift operator $\bbS$ and error matrix $\bbE$, $N$ is the size of spatial graph, and $T$ is the size of temporal graph.
\end{theorem}

\begin{proof}
	The difference between filter operators is
	\begin{equation}
		\bbH(\bbS_T,\hat{\bbS}) - \bbH(\bbS_T,\bbS) = \sum_{k=0}^{\infty}\sum_{l=0}^{\infty} h_{kl}[\bbS_T^l \otimes (\hat{\bbS}^k-\bbS^k)].
		\label{filterdiff}
	\end{equation}
	Since the spatial-temporal graph filters are permutation equivairant, without loss of generality, we can consider $\bbP = \bbI$. Hence, the difference between spatial shift operators can be reduced into the following first order Taylor expansion
	\begin{equation}
		\hat{\bbS}^k-\bbS^k = \sum_{r=0}^{k-1}(\bbS^r\bbE\bbS^{k-r}+\bbS^{r+1}\bbE\bbS^{k-r-1}) + \bbD
		\label{gsodiff}
	\end{equation}
	where $\bbD$ contains all the higher order terms in the expansion which are negligible \textcolor{red}{$\|\bbD\| = \ccalO(\eps^2)$}.
	
	Now, we assume an arbitrary signal over product graph $\bbx_\diamond$ with finite energy, i.e., $\|\bbx_\diamond\|<\infty$, to investigate the effect of perturbation on the output by calculating
	\begin{equation}
		\hat{\bby} - \bby = [\bbH(\bbS_T,\bbS) - \bbH(\bbS_T,\hat{\bbS})]\bbx_\diamond.
		\label{outputdiff}
	\end{equation}
	The signal $\bbx_\diamond$ has a spatial-temporal GFT of the form
	\begin{equation}
		\bbx_\diamond = \sum_{t=1}^{T}\sum_{i=1}^{N} \tilde{\bbx}_{ti} (\bbv_{Tt}\otimes\bbv_i).
		\label{GFT}
	\end{equation}
	Then, if we substitute $\bbx_\diamond$ in (\ref{outputdiff}) by its spatial-temporal GFT in (\ref{GFT}) and apply equations (\ref{filterdiff}) and (\ref{gsodiff}), we have
	\begin{align}
		[\bbH(\bbS_T,\bbS) &- \bbH(\bbS_T,\hat{\bbS})]\bbx_\diamond = \sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}\sum_{k=0}^{\infty}\sum_{l=0}^{\infty} h_{kl} \label{bigone}\\
		&[\bbS_T^l \otimes \sum_{r=0}^{k-1}(\bbS^r\bbE\bbS^{k-r}+\bbS^{r+1}\bbE\bbS^{k-r-1})] (\bbv_{Tt}\otimes\bbv_i) \nonumber
	\end{align}
	
	Now, we need to unravel the last term in (\ref{bigone}) to simplify it. To this end, first we use the well-known mixed-product property of Kronecker product
	$(\bbA \otimes \bbB)(\bbC \otimes \bbD) = (\bbA\bbC)\otimes(\bbB\bbD)$, so we have
	\begin{equation}
		\bbS_T^l\bbv_{Tt} \otimes \sum_{r=0}^{k-1}(\bbS^r\bbE\bbS^{k-r}+\bbS^{r+1}\bbE\bbS^{k-r-1})\bbv_i.
		\label{mixedproduct}
	\end{equation}
	 With the Eigenvalue definition, we can reduce (\ref{mixedproduct}) into
	 \begin{equation}
	 	\lambda_{Tt}^l\bbv_{Tt} \otimes \sum_{r=0}^{k-1}(\lambda_i^{k-r}\bbS^r+\lambda_i^{k-r-1}\bbS^{r+1})\bbE\bbv_i.
	 	\label{evreplaced}
	 \end{equation}
	 
	 To continue with the proof, we need the following lemma from \textcolor{red}{[Gamma2020]}
	 \begin{lemma}
	 	Let $\bbS=\bbV \bbLam \bbV^H$ and $\bbE = \bbU \bbM \bbU^H$ such that $\|\bbE\| \leq \eps$.
	 	For any eigenvector $\bbv_i$ of $\bbS$ it holds that
	 	\begin{equation}
	 		\bbE \bbv_i = m_i \bbv_i + \bbE_U \bbv_i
	 	\end{equation}
	 	with $\|\bbE_U\|\leq \eps\delta$, where $\delta = (\|\bbU -\bbV\|^2+1)^2-1$.
	 \end{lemma}
 	\textcolor{red}{Do I need to add some interpretation of this lemma?}
 	By applying this lemma on (\ref{evreplaced}) we now have
 	\begin{equation}
 		\lambda_{Tt}^l\bbv_{Tt} \otimes\sum_{r=0}^{k-1}2m_i\lambda_i^k\bbv_i +(\lambda_i^{k-r}\bbS^r+\lambda_i^{k-r-1}\bbS^{r+1})\bbE_U\bbv_i.
 		\label{lemmareplaced}
 	\end{equation}
	by replacing (\ref{lemmareplaced}) in (\ref{bigone}) we have
	\begin{align}
		[\bbH(&\bbS_T,\bbS) - \bbH(\bbS_T,\hat{\bbS})]\bbx_\diamond = \sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}\sum_{k=0}^{\infty}\sum_{l=0}^{\infty} h_{kl} \label{newbigone}\\
		&\lambda_{Tt}^l\bbv_{Tt} \otimes\sum_{r=0}^{k-1}2m_i\lambda_i^k\bbv_i +(\lambda_i^{k-r}\bbS^r+\lambda_i^{k-r-1}\bbS^{r+1})\bbE_U\bbv_i. \nonumber
	\end{align}
	
	For the first term we have
	\begin{equation}
		2\sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}m_i\sum_{k=0}^{\infty}\sum_{l=0}^{\infty} k h_{kl}\lambda_{Tt}^l\lambda_i^k (\bbv_{Tt}\otimes\bbv_i),
	\end{equation}
 	which can be simplified based on partial derivation definition
 	\begin{equation}
 		2\sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}m_i \lambda_i\frac{\partial h(\lambda_{Tt},\lambda_i)}{\partial \lambda_i} (\bbv_{Tt}\otimes\bbv_i).
 	\end{equation}
 	Assumptions (\ref{errorbound}) and (\ref{lipsch}) bound the norm of this term by $2C\eps\|\bbx_\diamond\|$.
 	
 	For the second term, we use mixed-product property again to separate different parts
 	\begin{align}
 		\sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}&(\bbI_T\otimes \bbV) 
 		(\bbI_T \otimes \diag(\bbg_i)) \label{secondterm} \\
 		&(\bbI_T\otimes \bbV^H)(\bbI_T\otimes \bbE_U) (\bbv_{Tt}\otimes\bbv_i), \nonumber
 	\end{align}
 	where 
 	\begin{align}
 		[\bbg_i]_j &= \sum_{k=0}^{\infty}\sum_{l=0}^{\infty} k h_{kl}\lambda_{Tt}^l\sum_{r=0}^{k-1}\lambda_i^{k-r}[\bbLambda^r]_j+\lambda_i^{k-r-1}[\bbLambda^{r+1}]_j \label{gdef} \\
 		&=\left\{
 		\begin{matrix}
 		&\lambda_i\frac{\partial h(\lambda_{Tt},\lambda_i)}{\partial \lambda_i} & \text{if}\quad i=j \\
 		&\frac{\lambda_i+\lambda_j}{\lambda_i-\lambda_j}(h(\lambda_{Tt},\lambda_i)-h(\lambda_{Tt},\lambda_j))&\text{if}\quad i=j
 		\end{matrix}
 		\right.. \nonumber
 	\end{align}
 	Based on integral Lipschitz functions definition, each entry of $\bbg_i$ is bounded by $2C$, hence the vector is bounded by $2C\sqrt{N}$.
 	Also $\bbI_T \otimes diag(\bbg_i)$ replicates the matrix for $T$ times so it is bounded by $2C\sqrt{NT}$.
 	Due to the Lemma. 1 $\|\bbE_U\|\leq \eps\delta$, and with the same reason, $\bbI_T \otimes \bbE_U$ is bounded by $\eps\delta\sqrt{T}$.
 	
 	All of the above bounds lead into the following equation
 	\begin{equation}
 		\|[\bbH(\bbS_T,\bbS) - \bbH(\bbS_T,\hat{\bbS})]\bbx_\diamond\| \leq 2C\eps(1+\delta T \sqrt{N}) \|\bbx_\diamond\|.
 	\end{equation}
 	So the proof is completed by assuming $\|\bbx_\diamond\| = 1$ as the definition.
 
 
 
 
\end{proof}

==> GTCNN paper/Sections/Spectral_proof.tex <==
Considering the graph-time filter in~\eqref{eq:graphtimegeneralfilter},  the input-output relation is
\begin{equation}
	\bby_{\diamond} =
	\sum_{k=0}^{\bar{K}}
	\sum_{l=0}^{\tilde{K}}
	h_{kl} (\bbS_T^l \otimes \bbS^k)
	\bbx_{\diamond}.
	\label{eq:input-output} 
\end{equation}
We apply graph-time Fourier transform by multiplying both sides with
$(\bbV_T\otimes\bbV)^H$
from left
\begin{equation}
	\tilde{\bby}_\diamond =
	\sum_{k=0}^{\bar{K}}
	\sum_{l=0}^{\tilde{K}}
	h_{kl}
	(\bbV_T\otimes\bbV)^H
	(\bbS_T^l \otimes \bbS^k)
	\bbx_{\diamond},	
\end{equation}
where
$\tilde{\bby}_\diamond$
is the graph-time Fourier transform of output $\bby_{\diamond}$.
Leveraging the mixed-product property of Kronecker product leads to
\begin{equation}
	\tilde{\bby}_\diamond =
	\sum_{k=0}^{\bar{K}}
	\sum_{l=0}^{\tilde{K}}
	h_{kl}
	(\bbV_T^H\bbS_T^l \otimes \bbV^H\bbS^k)
	\bbx_{\diamond}.
\end{equation}
Using eigenvalue decomposition we have
\begin{equation}
	\tilde{\bby}_\diamond =
	\sum_{k=0}^{\bar{K}}
	\sum_{l=0}^{\tilde{K}}
	h_{kl}
	(\bbLambda_T^l\bbV_T^H \otimes \bbLambda^k\bbV^H)
	\bbx_{\diamond}.
\end{equation}
Then, the Kronecker product property can be applied again
\begin{equation}
	\tilde{\bby}_\diamond =
	\sum_{k=0}^{\bar{K}}
	\sum_{l=0}^{\tilde{K}}
	h_{kl}
	(\bbLambda_T^l \otimes \bbLambda^k)
	(\bbV_T\otimes\bbV)^H
	\bbx_{\diamond}.
\end{equation}
The term
$(\bbV_T\otimes\bbV)^H\bbx_{\diamond}$ shows the graph-time Fourier transform of input $\bbx_{\diamond}$.
Hence we can complete the proof as
\begin{equation}
	\tilde{\bby}_\diamond = 
	h(\bbLambda_T,\bbLambda)
	\tilde{\bbx}_\diamond,
\end{equation}
where
\begin{equation}
	h(\bbLambda_T,\bbLambda) =
	\sum_{k=0}^{\bar{K}}
	\sum_{l=0}^{\tilde{K}}
	h_{kl}
	(\bbLambda_T^l \otimes \bbLambda^k)	.
\end{equation}

==> GTCNN paper/Sections/Stability.tex <==
We now investigate the stability properties of GTCNNs w.r.t. perturbations on the spatial graph to characterize its learning capabilities.
%While the spectral equivalence of graph-time convolutional filters tells us how each filter behaves in the layers, we here leverage such properties to study what are the effects of these filters in the stability of GTCNN to graph perturbations.
Analyzing stability is important as we often may not have access to the ground truth spatial graph.
In some cases, the inferred graph may be imperfect and we have to train the GTCNN over a perturbed graph;
in other cases, practical physical networks (e.g., water or power networks) slightly differ from the one we train the GTCNN, e.g., because of model mismatches.
So, having a stable GTCNN is desirable to perform the task reliably and allow transference~\cite{Ruiz2021GNN}.
%To this end, we define the essential concepts, then we use similar analysis as~\cite{gamamain}, and finally we will discuss the results.  

We analyze the stability w.r.t. the \emph{relative perturbation} over the spatial graph
\begin{equation}
	\hat{\bbS} = \bbS + (\bbE\bbS + \bbS\bbE)
	\label{relperturb}
\end{equation}
where $\hat{\bbS}$ is the perturbed GSO and $\bbE$ is the perturbation matrix~\cite{gamamain}.
Such model suggests that the graph perturbation depends on its structure, i.e., a node with more connected edges is relatively more prone to more perturbation.  
%So, relative perturbation model provides a realistic scenario for perturbation over networks.
%and it also builds a common ground to compare results with the work in~\cite{gamamain}.
%\red{EI: no need for this as a definition. Mention it inline as the perturbation model we consider, you also need to motivate it a bit why it is relevant and link it with Fernando's paper.}
To characterize the GTCNN stability,
%Next, we need to restrain the graph-time frequency response of the filters to analyze stability aspects of GTCNNs.
we consider graph-time convolutional filters with a frequency response that varies slightly in the high spatial frequencies (eigenvalues $\bbLambda$) and arbitrarily in the temporal one, see Fig.~\ref{fig:Lipschitz}. %This assumption is implied in the following definition. 
\begin{definition}
	\label{def:intlip}
	Given a graph-time filter with an analytic frequency response $h(\lambda_T,\lambda)$ [cf.~\eqref{eq:spectral}]. We say this filter is graph integral Lipschitz if there exists constant $C>0$ such that for all graph frequencies $\lambda_1,\lambda_2 \in \bbLambda$, it holds that
	\begin{equation}
		|h(\lambda_T,\lambda_2)-h(\lambda_T,\lambda_1)| \leq C \frac{|\lambda_2 - \lambda_1|}{|\lambda_2 + \lambda_1|/2}.
		\label{eq:lipmain}
	\end{equation}
\end{definition}
Expression~\eqref{eq:lipmain} implies that the filter's two-dimensional frequency response is Lipschitz in any interval $(\lambda_1, \lambda_2)$ of graph frequencies where the Lipschitz constant depends on their gap $|\lambda_2 + \lambda_1|/2$. The latter is similar to the integral Lipschitz property for GCNNs working on time invariant signals~\cite{gamamain} since we treat spatial perturbations, but it does not restrict the temporal behavior of the filter.%
\footnote{If we would ignore the product graph structure and discuss the stability results using~\cite{gamamain} straightforwardly the filter needed be spatiotemporal integral Lipschitz. This in turn affects discriminability~\cite{Ruiz2021GNN}.}
For the two-dimensional frequency response, this implies that its partial derivative is restricted as 
\begin{equation}
	\left|\lambda\frac{\partial h(\lambda_T,\lambda)}{\partial \lambda}\right| \leq C,	\label{eq:lipsch}
\end{equation}
i.e.,
%\red{EI: for this definition 2. It should be an assumption, no? You need then to intreoduce it as an assumption for characterizing the behavior of GTCNNs, also elaborate after what this assumption means and how it differs/generalizes the integral lipsitz filter; it also needs a 3D figure to illustrate it. Moreover, is the definition wrt. (16) or (17)? It should contain only one. I think (17) should be after the defitnition itself when you elaborate on it and motivate what this definition implies and why it is valid.}
the filters in a GTCNN have a frequency response that cannot vary drastically on high graph frequencies for all temporal frequencies but the filter can vary arbitrary over the temporal frequencies.
Fig.~\ref{fig:Lipschitz} illustrates this property.
%\blue{However, if we apply the results of~\cite{gamamain} directly on product graphs, they also restrain high temporal frequencies since that way we ignore the structure of product graph.} \red{This is discussion with Fernando's paper. First introduce your result and then discuss.} 

\begin{definition}
	\label{def:norm}
	Consider a graph-time convolutional filter with an analytic frequency response $h(\lambda_T,\lambda)$ [cf.~\eqref{eq:spectral}]. We say this filter has a normalized spectral response if $|h(\lambda_T,\lambda)| \leq 1$ for all $\lambda$, $\lambda_T$.
\end{definition}
This implies that the filter's gain $B = \|\bbH(\bbS_T,\bbS)\|$ to be less or equal to 1, $B\leq 1$, w.r.t. an $l_2$-measure.
Def.~\ref{def:norm} is required as the output of each layer should not magnify the input norm, otherwise, the system will become less stable as the number of layers increase, even in absence of perturbation.
Otherwise, constant $B$ would also appear in the following stability result of the GTCNN.

%With this in place, the following theorem proves GTCNN are stable to spatial perturbations.

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.7\linewidth]{Figures/Lipschitz.png}
	\caption{A spatial Lipschitz graph-time filter. The frequency response varies smoothly over high graph frequencies, while it has sudden changes on temporal frequencies.}
	\label{fig:Lipschitz}
\end{figure}

\begin{theorem}
	\label{filterstanility}
	Let $\bbS = \bbV\bbLambda\bbV^\herm$ and $\bbS_T\bbV_T\bbLambda_T\bbV_T^\herm$ be spatial and temporal graph shift operators, respectively.
	Let also $\hat{\bbS}$ be the relatively perturbed graph shift operator [cf.~\eqref{relperturb}].
	Consider the error matrix has the eigendecomposition
	$\bbE = \bbU \bbM \bbU^\herm$
	where $\bbU$ are the eigenvectors and $\bbM$ is the diagonal matrix of eigenvalues. Assume the error matrix has a bounded operator norm $\|\bbE\|\leq \eps.$
%	\begin{equation}
%	d(\bbS,\hat{\bbS}) \leq \|\bbE\|\leq \eps.
%	\label{errorbound}
%	\end{equation}
	Consider a GTCNN with L layers, F features and integral Lipschitz spatial-temporal graph filters [cf. Def.~\ref{def:intlip}] with normalized spectral responses [cf. Def.~\ref{def:norm}].
	Let also its nonlinearities be 1-Lipschitz, i.e., $|\sigma(a)-\sigma(b)| < |a-b|$, such as ReLU.
	Then, the distance between the GTCNN outputs $\Phi(\bbx_\diamond;\bbS_T,\bbS,\ccalH)$ on the nominal graph and $\Phi(\bbx_\diamond;\bbS_T,\hat{\bbS},\ccalH)$ on the perturbed graph is upper bounded by
	\begin{align}
	\|\Phi(\bbx_\diamond;\ccalH(\bbS_T,\bbS)) - \Phi(\bbx_\diamond;\ccalH(\bbS_T,\hat{\bbS})) \|_2 \leq LF^{L-1}\Delta\eps\|\bbx_\diamond\|_2
	\label{stabilitybound}
	\end{align}
	where $\Delta = 2C(1+\delta T\sqrt{N})$, $\delta = (\|\bbU-\bbV\|^2 +1)^2-1$ indicates the eigenvector misalignment between the spatial graph shift operator $\bbS$ and error matrix $\bbE$, $N$ is the size of spatial graph, and $T$ is the size of temporal graph.
\end{theorem}
\begin{proof}
	See Appendix~\ref{sec:stability_proof}.
\end{proof}

%%%%%%

Result~\eqref{stabilitybound} generalizes the findings in \cite{gamamain} to the spatiotemporal domain and states that GTCNNs are stable to relative perturbations in the spatial graph.
Together with the permutaiton equivariance~[Prop.~2], results~\eqref{stabilitybound} shows that GTCNNs allow for inductive learning and that are transferable architectures.
Such result provides three main insight on its stability/transferability:
%
\begin{enumerate}
\item The GTCNN is less stable for larger graphs ($\sqrt{N}$) as more nodes are exchanging information over a perturbed graph. Instead, its stability is more affected by the temporal resolution as increasing $T$ implies replicating the entire perturbed spatial graph.
\item The GTCNN is less stable if it is more discriminative in the nominal graph. This is reflected by term  $LF^{L-1}$ and it is due to the larger number of filters operating on the perturbed graphs. Such a observation shows also an inherit trade-off between stability and discriminability of GTCNNs.
\item Finally, we see the impact of each individual filter via the Lipschitz constant $C$. The latter in turn controls the filter discriminability on high graph frequencies to improve stability.
\end{enumerate}
%
%
%
%Result~\eqref{stabilitybound} states that the GTCNN is bounded w.r.t. relative perturbations in the spatial graph.
%The GTCNN is less stable if a larger temporal resolution $T$ is considered with a linear rate.
%This is because the perturbation replicates alongside with the spatial graph when the product graph is being made and $T$ controls the number of replica.
%The terms $LF^{L-1}$ is a design parameter that stands for the complexity of the model and indicates the number of graph-time convolutional filters.
%The model is less stable when it has more filters performing on a perturbed graph as the result~\eqref{stabilitybound} suggests.
%It also reflects a trade-off between discriminability and stability as a model with more filters and discriminability power is less stable.
%The second term $\Delta$ represents the stability of each individual filter.
%The integral Lipschitz constant $C$ controls the discriminability of each filter on high spatial graph frequencies and provides another design opportunity to compromise between discriminability and stability.
%The part $\delta\sqrt{N}$ measures the spatial eigenvector misalignment and it is ruled by the problem.
%The model is less stable for larger graphs as more nodes are exchanging information over a perturbed graph.
%Finally, $T$ replicates the eigenvector misalignment caused by perturbation over the product graph and the model is less stable if there are more replica of perturbed spatial graph.



%\red{
%There is one observation unaddressed.
%Why T effect is more severe than N.
%I know the answer in math but cannot phrase it.
%}



\smallskip
\noindent\textbf{Comparison with alternative bounds.} We discuss now that exploring the product graph sparsity with GTCNN provides more stable solutions compared with baselines that ignore it.
We discuss also the relation of result \eqref{stabilitybound} with the stability result for spatiotemporal learning~\cite{mo:ruiz2020gatedGRNN,hadou2021space}.

%Theorem~\ref{filterstanility}
%provides a stability bound for learning spatiotemporal representations with the GTCNN. However, we could also operate differently on the data and use existing stability results. Here, we discuss the relations between result~\eqref{stabilitybound} and alternatives.
%guarantees that GTCNN are stable to spatial relative perturbations and provides insights on the role played by the different architecture components. We can also approach the problem of learning from spatiotemporal relations with different GNN-based solution and leverage existing bound results. We here discuss the implications of bound~\eqref{stabilitybound} w.r.t. two alternatives: GCNN over product graph and multiple feature GCNN.

%To compare our results with previous works, we can translate multivariate temporal data for GCNNs.
\smallskip
\emph{Product graph GCNN:} One trivial learning solution on product graphs is to ignore what different edges represent and naively deploy a GCNN over this large graph of $NT$ nodes. Using the results in
%We can consider the product graph as a large graph of $NT$ nodes, the temporal data as static over this graph, and use directly the GCNN~\cite{gama2020elvinmagazine} to learn representations.
%Employing the results from
~\cite{gamamain}, such GCNN has a stability bound $\Delta_\text{GCNN} = 2C\sqrt{T}(1+\delta\sqrt{NT})$ since it assumes the perturbation over all the edges in the product graph including temporal ones, so, the noise energy scales by $\sqrt{T}$ and it applies over $NT$ nodes.
%ignores any temporal dependencies in the theoretical analysis and assumes the perturbation over all the edges in the product graph including temporal ones, so it is not a proper analysis.
The latter leads to a stability bound $2CT$ times looser than~\eqref{stabilitybound}.
Moreover, Theorem~\ref{filterstanility} restrains the graph-time filter variability only on spatial frequencies, while if we apply directly the results of~\cite{gamamain}, we restrain also high temporal frequency variations.
%Comparing this result with~\eqref{stabilitybound}, one can notice a gap between the bounds $\Delta_\text{GCNN}-\Delta_\text{GTCNN} = 2CT$.
%This gap is considerable since it varies linearly by the number of timestamps $T$.
%So, if we ignore the special structure of product graphs, a GCNN for a graph with $NT$ nodes or a graph data with $N$ nodes and $T$ features have at least a stability bound $\sqrt{T}$ times looser.


\smallskip
\emph{GCNNs:}
Another way to approach spatiotemporal learning is to treat the time series as features over the nodes and deploy a conventional GCNN. Leveraging again the result of~\cite{gamamain}, such a solution will have a stability bound $\Delta_\text{GCNN} = 2CT^L(1+\delta\sqrt{N})$ as we replicate filters in each layer $T$ times for each feature, including the input layer.
This bound is magnificently large due to factor $T^L$.
%This bound forms because of the rise in the number of filters appeared in the model to process data over $T$ input features. 


\smallskip
\emph{GGRNN~\cite{mo:ruiz2020gatedGRNN}:}
Graph gated recurrent neural networks (GGRNNs) replace the linear transformations in a recurrent neural network with graph filters to learn spatiotemporal patterns. They have a stability bound $\Delta_{\text{GGRNN}} = C(1+\sqrt{N}\delta)(T^2+3T)$. %for a time series of fixed length $T$.
Comparing with~\eqref{stabilitybound}, $\Delta_{\text{GGRNN}}$ expands at a higher rate by a factor of $T$, but note that the term $T^2+3T$ also implicitly contains the effect of layers $L$ in itself.
The assumptions behind the stability theorem in~\cite{mo:ruiz2020gatedGRNN} are similar to Theorem~\ref{filterstanility}, i.e., spatial integral Lipschitz filters and 1-Lipschitz nonlinearity.
%except an extra assumption that restricts input multivariate time series to be normalized over timestamps $\|\bbx_t\|\leq 1$.
In conclusion, Theorem~\ref{filterstanility} and~\cite{mo:ruiz2020gatedGRNN} present closely related stability bounds based similar conditions but for different models.


\smallskip
\emph{ST-GNN~\cite{hadou2021space}:}
Space-time graph neural network (ST-GNN) linearly composes a GSO with a continuous time shift operator to define a space-time shift operator.
%Space-time convolution uses such expanded shift operator to diffuse spatiotemporal information.
%They studied the stability to both temporal and spatial relative perturbations.
The stability to relative perturbation on the spatial graph is equal to GCNN~\cite{gama2020elvinmagazine}, i.e., $\Delta_{\text{STGNN}} = 2C(1+\delta\sqrt{N}) $.
This bound suggests that ST-GNN can process temporal properties of times series robustly under spatial perturbation.
The result~\eqref{stabilitybound} reflects the effect of time series length on stability of GTCNN as it involves time directly into convolutional filters to capture spatiotemporal patterns in the data.



%To summarize, our result suggests that if we consider the product graph structure there will be notably less limitations on graph-time filters frequency response and approves that GTCNNs can have better performance while holding the stability.
%\textcolor{red}{if I start the proof here, the lemma will be in the proof.}
%To prove this theorem, we followed the same procedure as~\cite{gamamain} and the following lemma is required to complete the proof
%\begin{lemma}(see~\cite{gamamain})
%	Let $\bbS=\bbV \bbLam \bbV^H$ and $\bbE = \bbU \bbM \bbU^H$ such that $\|\bbE\| \leq \eps$.
%	For any eigenvector $\bbv_i$ of $\bbS$ it holds that
%	\begin{equation}
%	\bbE \bbv_i = m_i \bbv_i + \bbE_U \bbv_i
%	\end{equation}
%	with $\|\bbE_U\|\leq \eps\delta$, where $\delta = (\|\bbU -\bbV\|^2+1)^2-1$.
%	\label{mainlemma}
%\end{lemma}
%
%\begin{proof}
%	The difference between filter operators is
%	\begin{equation}
%	\bbH(\bbS_T,\hat{\bbS}) - \bbH(\bbS_T,\bbS) = \sum_{k=0}^{\infty}\sum_{l=0}^{\infty} h_{kl}[\bbS_T^l \otimes (\hat{\bbS}^k-\bbS^k)].
%	\label{filterdiff}
%	\end{equation}
%	Since the spatial-temporal graph filters are permutation equivairant, without loss of generality, we can consider $\bbP = \bbI$. Hence, the difference between spatial shift operators can be reduced into the following first order Taylor expansion
%	\begin{equation}
%	\hat{\bbS}^k-\bbS^k = \sum_{r=0}^{k-1}(\bbS^r\bbE\bbS^{k-r}+\bbS^{r+1}\bbE\bbS^{k-r-1}) + \bbD
%	\label{gsodiff}
%	\end{equation}
%	where $\bbD$ contains all the higher order terms in the expansion which are negligible.
%	
%	Now, we assume an arbitrary signal over product graph $\bbx_\diamond$ with finite energy, i.e., $\|\bbx_\diamond\|<\infty$, to investigate the effect of perturbation on the output by calculating
%	\begin{equation}
%	\hat{\bby} - \bby = [\bbH(\bbS_T,\bbS) - \bbH(\bbS_T,\hat{\bbS})]\bbx_\diamond.
%	\label{outputdiff}
%	\end{equation}
%	The signal $\bbx_\diamond$ has a spatial-temporal GFT of the form
%	\begin{equation}
%	\bbx_\diamond = \sum_{t=1}^{T}\sum_{i=1}^{N} \tilde{\bbx}_{ti} (\bbv_{Tt}\otimes\bbv_i).
%	\label{GFT}
%	\end{equation}
%	Then, if we substitute $\bbx_\diamond$ in (\ref{outputdiff}) by its spatial-temporal GFT in (\ref{GFT}) and apply equations (\ref{filterdiff}) and (\ref{gsodiff}), we have
%	\begin{align}
%	[\bbH(\bbS_T,\bbS) &- \bbH(\bbS_T,\hat{\bbS})]\bbx_\diamond = \sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}\sum_{k=0}^{\infty}\sum_{l=0}^{\infty} h_{kl} \label{bigone}\\
%	&[\bbS_T^l \otimes \sum_{r=0}^{k-1}(\bbS^r\bbE\bbS^{k-r}+\bbS^{r+1}\bbE\bbS^{k-r-1})] (\bbv_{Tt}\otimes\bbv_i) \nonumber
%	\end{align}
%	
%	Now, we need to unravel the last term in (\ref{bigone}) to simplify it. To this end, first we use the well-known mixed-product property of Kronecker product
%	$(\bbA \otimes \bbB)(\bbC \otimes \bbD) = (\bbA\bbC)\otimes(\bbB\bbD)$, so we have
%	\begin{equation}
%	\bbS_T^l\bbv_{Tt} \otimes \sum_{r=0}^{k-1}(\bbS^r\bbE\bbS^{k-r}+\bbS^{r+1}\bbE\bbS^{k-r-1})\bbv_i.
%	\label{mixedproduct}
%	\end{equation}
%	With the Eigenvalue definition, we can reduce (\ref{mixedproduct}) into
%	\begin{equation}
%	\lambda_{Tt}^l\bbv_{Tt} \otimes \sum_{r=0}^{k-1}(\lambda_i^{k-r}\bbS^r+\lambda_i^{k-r-1}\bbS^{r+1})\bbE\bbv_i.
%	\label{evreplaced}
%	\end{equation}
%	
%	By applying Lemma.~\ref{mainlemma} on (\ref{evreplaced}) we now have
%	\begin{equation}
%	\lambda_{Tt}^l\bbv_{Tt} \otimes\sum_{r=0}^{k-1}2m_i\lambda_i^k\bbv_i +(\lambda_i^{k-r}\bbS^r+\lambda_i^{k-r-1}\bbS^{r+1})\bbE_U\bbv_i.
%	\label{lemmareplaced}
%	\end{equation}
%	by replacing (\ref{lemmareplaced}) in (\ref{bigone}) we have
%	\begin{align}
%	[\bbH(&\bbS_T,\bbS) - \bbH(\bbS_T,\hat{\bbS})]\bbx_\diamond = \sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}\sum_{k=0}^{\infty}\sum_{l=0}^{\infty} h_{kl} \label{newbigone}\\
%	&\lambda_{Tt}^l\bbv_{Tt} \otimes\sum_{r=0}^{k-1}2m_i\lambda_i^k\bbv_i +(\lambda_i^{k-r}\bbS^r+\lambda_i^{k-r-1}\bbS^{r+1})\bbE_U\bbv_i. \nonumber
%	\end{align}
%	
%	For the first term we have
%	\begin{equation}
%	2\sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}m_i\sum_{k=0}^{\infty}\sum_{l=0}^{\infty} k h_{kl}\lambda_{Tt}^l\lambda_i^k (\bbv_{Tt}\otimes\bbv_i),
%	\end{equation}
%	which can be simplified based on partial derivation definition
%	\begin{equation}
%	2\sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}m_i \lambda_i\frac{\partial h(\lambda_{Tt},\lambda_i)}{\partial \lambda_i} (\bbv_{Tt}\otimes\bbv_i).
%	\end{equation}
%	Assumptions (\ref{errorbound}) and (\ref{lipsch}) bound the norm of this term by $2C\eps\|\bbx_\diamond\|$.
%	
%	For the second term, we use mixed-product property again to separate different parts
%	\begin{align}
%	\sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}&(\bbI_T\otimes \bbV) 
%	(\bbI_T \otimes \diag(\bbg_i)) \label{secondterm} \\
%	&(\bbI_T\otimes \bbV^H)(\bbI_T\otimes \bbE_U) (\bbv_{Tt}\otimes\bbv_i), \nonumber
%	\end{align}
%	where 
%	\begin{align}
%	[\bbg_i]_j &= \sum_{k=0}^{\infty}\sum_{l=0}^{\infty} k h_{kl}\lambda_{Tt}^l\sum_{r=0}^{k-1}\lambda_i^{k-r}[\bbLambda^r]_j+\lambda_i^{k-r-1}[\bbLambda^{r+1}]_j \label{gdef} \\
%	&=\left\{
%	\begin{matrix}
%	&\lambda_i\frac{\partial h(\lambda_{Tt},\lambda_i)}{\partial \lambda_i} & \text{if}\quad i=j \\
%	&\frac{\lambda_i+\lambda_j}{\lambda_i-\lambda_j}(h(\lambda_{Tt},\lambda_i)-h(\lambda_{Tt},\lambda_j))&\text{if}\quad i=j
%	\end{matrix}
%	\right.. \nonumber
%	\end{align}
%	Based on integral Lipschitz functions definition, each entry of $\bbg_i$ is bounded by $2C$, hence the vector is bounded by $2C\sqrt{N}$.
%	Also $\bbI_T \otimes diag(\bbg_i)$ replicates the matrix for $T$ times so it is bounded by $2C\sqrt{NT}$.
%	Due to the Lemma. 1 $\|\bbE_U\|\leq \eps\delta$, and with the same reason, $\bbI_T \otimes \bbE_U$ is bounded by $\eps\delta\sqrt{T}$.
%	
%	All of the above bounds lead into the following equation
%	\begin{equation}
%	\|[\bbH(\bbS_T,\bbS) - \bbH(\bbS_T,\hat{\bbS})]\bbx_\diamond\| \leq 2C\eps(1+\delta T \sqrt{N}) \|\bbx_\diamond\|.
%	\end{equation}
%	So the proof is completed by assuming $\|\bbx_\diamond\| = 1$.
%\end{proof}
%
%\begin{theorem}
%	Let $\bbS$ and $\hat{\bbS}$ be GSOs related by relative perturbation matrix $\bbE$ as in~(\ref{relperturb}) such that $\|\bbE\|<\eps$.
%	Consider all filters in the GTCNN satisfy the assumptions in Theorem.~\ref{filterstanility} and point-wise nonlinearities are Lipschitz continuous.
%	Then it holds that
%	\begin{equation}
%		\|\Phi(\bbS,\cdot) - \Phi(\hat{\bbS},\cdot)\|\bbx_\diamond \leq 2CLF^{(L-1)}(1+\delta T \sqrt{N})\eps\|\bbx_\diamond\|
%	\end{equation}
%	for a GTCNN with $L$ layers and $F$ features in each hidden layer.
%	
%\end{theorem}

%\textcolor{red}{I need a bit time for this part, I am already working on some different scenarios to compare the bounds.}

==> GTCNN paper/Sections/gtfilter_proof.tex <==
The graph time convolutional filter in~\eqref{eq:graphtimefilter} operating over the parametric product graph is
\begin{equation}
	\bby_\diamond = \sum_{k=0}^K h_k \left(\sum_{i = 0}^1 \sum_{j = 0}^1 s_{ij}  \left(\mathbf{S}_{T}^{i} \otimes  \mathbf{S}^{j}  \right)\right)^k \bbx_\diamond.
	\label{eq:paramgtfilter}
\end{equation}
To expand equation~\eqref{eq:paramgtfilter}, we first investigate the powers of the parametric product graph
\begin{equation}
	\bbS_\diamond^k =
	(s_{00}\bbI_T\otimes\bbI_N+
	s_{01}\bbI_T\otimes\bbS+
	s_{10}\bbS_T\otimes\bbI_N+
	s_{11}\bbS_T\otimes\bbS_N)^k.
	\label{eq:powers} 
\end{equation}
Equation~\eqref{eq:powers} is expandable by multinomial theorem. The expanded version after applying mixed-product property of Kronecker product is
\begin{align}
	&\sum_{\mathclap{\sum k_{ij} = k}}c_\ccalI(\bbI_T\otimes\bbI_N)^{k_{00}}
	(\bbI_T\otimes\bbS)^{k_{01}}
	(\bbS_T\otimes\bbI_N)^{k_{10}}
	(\bbS_T\otimes\bbS_N)^{k_{11}}
	\nonumber \\
	&= \sum_{\mathclap{\sum k_{ij} = k}}c_\ccalI(\bbS_T^{k_{10}+k_{11}}\otimes\bbS^{k_{01}+k_{11}})
	\label{eq:powersexpanded}
\end{align}
where $\ccalI = \{k_{00},k_{01},k_{10},k_{11}\}$ is the multinomial term index and $c_\ccalI$ is the respective term coefficient.

Substituting the parametric graph powers~\eqref{eq:powersexpanded} into the parametric graph time convolutional filter~\eqref{eq:paramgtfilter} leads to
\begin{equation}
	\bby_\diamond = \sum_{k=0}^K h_k
	\sum_{k_{00}+k_{01}+k_{10}+k_{11} = k}c_\ccalI(\bbS_T^{k_{10}+k_{11}}\otimes\bbS^{k_{01}+k_{11}})
	\bbx_\diamond.
	\label{eq:doublesum}
\end{equation}
By a change of variables $l=k_{10}+k_{11}$ and $p=k_{01}+k_{11}$, we reduce~\eqref{eq:doublesum} into
\begin{equation}
	\bby_\diamond = \sum_{k=0}^K h_k
	\sum_{l+p = k}c_{lp}(\bbS_T^{l}\otimes\bbS^{p})
	\bbx_\diamond.
	\label{tmp10}
\end{equation}
By further changing the indexing and order of summation we can write~\eqref{tmp10} as
\begin{equation}
	\bby_\diamond = \sum_{l=0}^{K}\sum_{p=0}^{K-l} h_{lp}c_{lp}(\bbS_T^{l}\otimes\bbS^{p})
	\bbx_\diamond.
	\label{tmp11}
\end{equation}
Hence, the graph time convolutional filter in~\eqref{eq:paramgtfilter} is equivalent to~\eqref{tmp11}, which in turn is a specific case of~\eqref{eq:graphtimegeneralfilter} with $\bar{K} = K - l$, $\tilde{K} = K$, and $h_{kl} = h_{lp}c_{lp}$.

%The multinomial coefficients can be calculated by
%\begin{equation}
%	c_\ccalI = 
%	\left(\begin{matrix}
%		k \\
%		k_{00},k_{01},k_{10},k_{11}
%	\end{matrix}\right)
%	\prod_{i=0}^{1}\prod_{j=0}^{1} s_{ij}^{k_{ij}}
%\end{equation}
%with
%\begin{equation}
%	\left(\begin{matrix}
%		k \\
%		k_{00},k_{01},k_{10},k_{11}
%	\end{matrix}\right) =
%	\frac{k!}{k_{00}!k_{01}!k_{10}!k_{11}!},
%\end{equation}
%and $c_{lp}$ collects them over specific powers $l$ and $p$
%\begin{equation}
%	c_{lp} = \sum_{\substack{k_{10} + K_{11} = l \\ k_{01} + K_{11} = p}} c_\ccalI.
%\end{equation}

==> GTCNN paper/mySections.tex <==
\usepackage{needspace}

% \nbsubsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsubsection}[1]{\needspace{1\baselineskip}\color{white}\subsubsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsubsection. #1.}}

% \myparagraph provides a paragraph title in italics. 
\newcommand{\myparagraph}[1]{\needspace{1\baselineskip}\medskip\noindent {\bf #1}}

% \myindenetedparagraph provides an indented paragraph with title in italics.
\newcommand{\myindentedparagraph}[1]{\needspace{1\baselineskip}\medskip \hangindent=11pt \hangafter=0 \noindent{\it #1.}}

% \myparagraphtc provides a paragraph title in italics. It adds an enter to the table of contents
\newcommand{\myparagraphtc}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}\addcontentsline{toc}{subsubsection}{\qquad\qquad\quad#1}}



==> Sections/Proof.tex <==
\begin{theorem}
	Let $\bbS = \bbV\Lambda\bbV^H$ and $\bbS_T\bbV_T\Lambda_T\bbV_T^H$ be spatial and temporal graph shift operators respectively.
	Assume $\hat{\bbS}$ is the relatively perturbed graph shift operator, i.e., $\bbP^\top\hat{\bbS}\bbP = \bbS + (\bbE\bbS + \bbS\bbE)$ where $\bbP$ is a permutation matrix and $\bbE = \bbU \bbM \bbU^H \in \ccalE(\bbS,\hat{\bbS})$ is the error matrix with a bounded norm
	\begin{equation}
		d(\bbS,\hat{\bbS}) \leq \|\bbE\|\leq \eps.
		\label{errorbound}
	\end{equation}
	For an integral Lipschitz spatial-temporal graph filter with respect to spatial eigenvalues
	\begin{equation}
		\lambda \frac{\partial h(\lambda_T,\lambda)}{\partial \lambda} \leq C
		\label{lipsch}
	\end{equation}
	the operator distance modulo permutation between filters $\bbH(\bbS_T,\bbS)$ and $\bbH(\bbS_T,\hat{\bbS})$ satisfies
	\begin{equation}
		\|\bbH(\bbS_T,\bbS) - \bbH(\bbS_T,\hat{\bbS}) \|_\ccalP \leq 2C\eps(1+T\delta \sqrt{NT}) + \ccalO(\eps^2)
	\end{equation}
	where $\delta = (\|\bbU-\bbV\|_2 +1)^2-1$ indicates the eigenvector misalignment between the spatial graph shift operator $\bbS$ and error matrix $\bbE$, $N$ is the size of spatial graph, and $T$ is the size of temporal graph.
\end{theorem}

\begin{proof}
	The difference between filter operators is
	\begin{equation}
		\bbH(\bbS_T,\hat{\bbS}) - \bbH(\bbS_T,\bbS) = \sum_{k=0}^{\infty}\sum_{l=0}^{\infty} h_{kl}[\bbS_T^l \otimes (\hat{\bbS}^k-\bbS^k)].
		\label{filterdiff}
	\end{equation}
	Since the spatial-temporal graph filters are permutation equivairant, without loss of generality, we can consider $\bbP = \bbI$. Hence, the difference between spatial shift operators can be reduced into the following first order Taylor expansion
	\begin{equation}
		\hat{\bbS}^k-\bbS^k = \sum_{r=0}^{k-1}(\bbS^r\bbE\bbS^{k-r}+\bbS^{r+1}\bbE\bbS^{k-r-1}) + \bbD
		\label{gsodiff}
	\end{equation}
	where $\bbD$ contains all the higher order terms in the expansion which are negligible \textcolor{red}{$\|\bbD\| = \ccalO(\eps^2)$}.
	
	Now, we assume an arbitrary signal over product graph $\bbx_\diamond$ with finite energy, i.e., $\|\bbx_\diamond\|<\infty$, to investigate the effect of perturbation on the output by calculating
	\begin{equation}
		\hat{\bby} - \bby = [\bbH(\bbS_T,\bbS) - \bbH(\bbS_T,\hat{\bbS})]\bbx_\diamond.
		\label{outputdiff}
	\end{equation}
	The signal $\bbx_\diamond$ has a spatial-temporal GFT of the form
	\begin{equation}
		\bbx_\diamond = \sum_{t=1}^{T}\sum_{i=1}^{N} \tilde{\bbx}_{ti} (\bbv_{Tt}\otimes\bbv_i).
		\label{GFT}
	\end{equation}
	Then, if we substitute $\bbx_\diamond$ in (\ref{outputdiff}) by its spatial-temporal GFT in (\ref{GFT}) and apply equations (\ref{filterdiff}) and (\ref{gsodiff}), we have
	\begin{align}
		[\bbH(\bbS_T,\bbS) &- \bbH(\bbS_T,\hat{\bbS})]\bbx_\diamond = \sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}\sum_{k=0}^{\infty}\sum_{l=0}^{\infty} h_{kl} \label{bigone}\\
		&[\bbS_T^l \otimes \sum_{r=0}^{k-1}(\bbS^r\bbE\bbS^{k-r}+\bbS^{r+1}\bbE\bbS^{k-r-1})] (\bbv_{Tt}\otimes\bbv_i) \nonumber
	\end{align}
	
	Now, we need to unravel the last term in (\ref{bigone}) to simplify it. To this end, first we use the well-known mixed-product property of Kronecker product
	$(\bbA \otimes \bbB)(\bbC \otimes \bbD) = (\bbA\bbC)\otimes(\bbB\bbD)$, so we have
	\begin{equation}
		\bbS_T^l\bbv_{Tt} \otimes \sum_{r=0}^{k-1}(\bbS^r\bbE\bbS^{k-r}+\bbS^{r+1}\bbE\bbS^{k-r-1})\bbv_i.
		\label{mixedproduct}
	\end{equation}
	 With the Eigenvalue definition, we can reduce (\ref{mixedproduct}) into
	 \begin{equation}
	 	\lambda_{Tt}^l\bbv_{Tt} \otimes \sum_{r=0}^{k-1}(\lambda_i^{k-r}\bbS^r+\lambda_i^{k-r-1}\bbS^{r+1})\bbE\bbv_i.
	 	\label{evreplaced}
	 \end{equation}
	 
	 To continue with the proof, we need the following lemma from \textcolor{red}{[Gamma2020]}
	 \begin{lemma}
	 	Let $\bbS=\bbV \bbLam \bbV^H$ and $\bbE = \bbU \bbM \bbU^H$ such that $\|\bbE\| \leq \eps$.
	 	For any eigenvector $\bbv_i$ of $\bbS$ it holds that
	 	\begin{equation}
	 		\bbE \bbv_i = m_i \bbv_i + \bbE_U \bbv_i
	 	\end{equation}
	 	with $\|\bbE_U\|\leq \eps\delta$, where $\delta = (\|\bbU -\bbV\|^2+1)^2-1$.
	 \end{lemma}
 	\textcolor{red}{Do I need to add some interpretation of this lemma?}
 	By applying this lemma on (\ref{evreplaced}) we now have
 	\begin{equation}
 		\lambda_{Tt}^l\bbv_{Tt} \otimes\sum_{r=0}^{k-1}2m_i\lambda_i^k\bbv_i +(\lambda_i^{k-r}\bbS^r+\lambda_i^{k-r-1}\bbS^{r+1})\bbE_U\bbv_i.
 		\label{lemmareplaced}
 	\end{equation}
	by replacing (\ref{lemmareplaced}) in (\ref{bigone}) we have
	\begin{align}
		[\bbH(&\bbS_T,\bbS) - \bbH(\bbS_T,\hat{\bbS})]\bbx_\diamond = \sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}\sum_{k=0}^{\infty}\sum_{l=0}^{\infty} h_{kl} \label{newbigone}\\
		&\lambda_{Tt}^l\bbv_{Tt} \otimes\sum_{r=0}^{k-1}2m_i\lambda_i^k\bbv_i +(\lambda_i^{k-r}\bbS^r+\lambda_i^{k-r-1}\bbS^{r+1})\bbE_U\bbv_i. \nonumber
	\end{align}
	
	For the first term we have
	\begin{equation}
		2\sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}m_i\sum_{k=0}^{\infty}\sum_{l=0}^{\infty} k h_{kl}\lambda_{Tt}^l\lambda_i^k (\bbv_{Tt}\otimes\bbv_i),
	\end{equation}
 	which can be simplified based on partial derivation definition
 	\begin{equation}
 		2\sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}m_i \lambda_i\frac{\partial h(\lambda_{Tt},\lambda_i)}{\partial \lambda_i} (\bbv_{Tt}\otimes\bbv_i).
 	\end{equation}
 	Assumptions (\ref{errorbound}) and (\ref{lipsch}) bound the norm of this term by $2C\eps\|\bbx_\diamond\|$.
 	
 	For the second term, we use mixed-product property again to separate different parts
 	\begin{align}
 		\sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}&(\bbI_T\otimes \bbV) 
 		(\bbI_T \otimes \diag(\bbg_i)) \label{secondterm} \\
 		&(\bbI_T\otimes \bbV^H)(\bbI_T\otimes \bbE_U) (\bbv_{Tt}\otimes\bbv_i), \nonumber
 	\end{align}
 	where 
 	\begin{align}
 		[\bbg_i]_j &= \sum_{k=0}^{\infty}\sum_{l=0}^{\infty} k h_{kl}\lambda_{Tt}^l\sum_{r=0}^{k-1}\lambda_i^{k-r}[\bbLambda^r]_j+\lambda_i^{k-r-1}[\bbLambda^{r+1}]_j \label{gdef} \\
 		&=\left\{
 		\begin{matrix}
 		&\lambda_i\frac{\partial h(\lambda_{Tt},\lambda_i)}{\partial \lambda_i} & \text{if}\quad i=j \\
 		&\frac{\lambda_i+\lambda_j}{\lambda_i-\lambda_j}(h(\lambda_{Tt},\lambda_i)-h(\lambda_{Tt},\lambda_j))&\text{if}\quad i=j
 		\end{matrix}
 		\right.. \nonumber
 	\end{align}
 	Based on integral Lipschitz functions definition, each entry of $\bbg_i$ is bounded by $2C$, hence the vector is bounded by $2C\sqrt{N}$.
 	Also $\bbI_T \otimes diag(\bbg_i)$ replicates the matrix for $T$ times so it is bounded by $2C\sqrt{NT}$.
 	Due to the Lemma. 1 $\|\bbE_U\|\leq \eps\delta$, and with the same reason, $\bbI_T \otimes \bbE_U$ is bounded by $\eps\delta\sqrt{T}$.
 	
 	All of the above bounds lead into the following equation
 	\begin{equation}
 		\|[\bbH(\bbS_T,\bbS) - \bbH(\bbS_T,\hat{\bbS})]\bbx_\diamond\| \leq 2C\eps(1+\delta T \sqrt{N}) \|\bbx_\diamond\|.
 	\end{equation}
 	So the proof is completed by assuming $\|\bbx_\diamond\| = 1$ as the definition.
 
 
 
 
\end{proof}

==> Sections/stability_proof.tex <==
The proof follows closely as that for the GCNNs in~\cite{gamamain}, but the product graph requires a few changes. We will also use the following lemma. 
\begin{lemma}[c.f.~\cite{gamamain}]
	Let $\bbS=\bbV \bbLam \bbV^\herm$ and $\bbE = \bbU \bbM \bbU^\herm$ such that $\|\bbE\| \leq \eps$.
	Assume that $\bbE_V = \bbV \bbM \bbV^\herm$ is the projection of perturbation $\bbE$ over graph eigenspace, and $\bbE = \bbE_V+\bbE_U$.
	For any eigenvector $\bbv_i$ of $\bbS$ it holds that
	\begin{equation}
		\bbE \bbv_i = m_i \bbv_i + \bbE_U \bbv_i
		\end{equation}
	with $\|\bbE_U\|\leq \eps\delta$, where $\delta = (\|\bbU -\bbV\|^2+1)^2-1$ and $m_i$ is the $i$-th eigenvalue of $\bbM$.
	Recall that $\|\cdot\|$ represents the operator norm of a matrix.
	\label{mainlemma}
\end{lemma}

The proof is organized into two parts. First, we prove graph-time convolutional filter [cf.~\eqref{eq:graphtimegeneralfilter}] is stable and then we extend it to the GTCNN.

\smallskip
\noindent\textbf{Filter.}
Let $\bbx_\diamond$ be the input signal over product graph with finite energy, i.e., $\|\bbx_\diamond\|_2<\infty$.
The effect of perturbation on the output is
\begin{equation}
	\| \hat{\bby} - \bby \|_2 = \left\| [\bbH(\bbS_T,\bbS) - \bbH(\bbS_T,\hat{\bbS})]\bbx_\diamond\right\|_2.
	\label{outputdiff}
\end{equation}
The difference between convolutional filter operators can be further written as
\begin{equation}
	\bbH(\bbS_T,\hat{\bbS}) - \bbH(\bbS_T,\bbS) = \sum_{k=0}^{\bar{K}}\sum_{l=0}^{\tilde{K}} h_{kl}[\bbS_T^l \otimes (\hat{\bbS}^k-\bbS^k)].
	\label{filterdiff}
	\end{equation}
%Since the spatial-temporal graph filters are permutation equivairant, without loss of generality, we can consider $\bbP = \bbI$.
As in~\eqref{filterdiff}, we discussed the case for filters of orders infinity which allows us to link these discrete filters to their continuous spectral response.
%This will loose the bound yet we need it for the sake of theoretical analysis.
The difference between spatial shift operators, $\bbS$ and $\hat{\bbS}$, can be expanded by first-order Taylor series approximation as
\begin{equation}
	\hat{\bbS}^k-\bbS^k = \sum_{r=0}^{k-1}(\bbS^r\bbE\bbS^{k-r}+\bbS^{r+1}\bbE\bbS^{k-r-1}) + \bbD
	\label{gsodiff}
	\end{equation}
where $\bbD = \ccalO(\eps^2)$ is negligible.

With this in place, we now move to the spectral domain. The graph-time Fourier decomposition for the signal $\bbx_\diamond$ over the product graph is
\begin{equation}
	\bbx_\diamond =  (\bbV_T \otimes \bbV)\tilde{\bbx}_{\diamond} = \sum_{t=1}^{T}\sum_{i=1}^{N} \tilde{\bbx}_{ti} (\bbv_{T,t}\otimes\bbv_i).
	\label{GFT}
\end{equation}
%which indicates the signal variations on both time and space.
Substituting expansion~\eqref{GFT} of $\bbx_\diamond$ and~(\ref{gsodiff}) into~(\ref{outputdiff}), we have
\begin{align}
	\| \hat{\bby} - \bby \|&_2= \left\| \sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}\sum_{k=0}^{\bar{K}}\sum_{l=0}^{\tilde{K}} h_{kl} \label{bigone}\right.\\
	&\left. [\bbS_T^l \otimes \sum_{r=0}^{k-1}(\bbS^r\bbE\bbS^{k-r}+\bbS^{r+1}\bbE\bbS^{k-r-1})] (\bbv_{Tt}\otimes\bbv_i) \right\|_2 \nonumber
\end{align}

Now, we expand the inner summation in (\ref{bigone}) to simplify it. By using the mixed-product property of Kronecker product
$(\bbA \otimes \bbB)(\bbC \otimes \bbD) = (\bbA\bbC)\otimes(\bbB\bbD)$, we have
\begin{align}
	 &[\bbS_T^l \otimes \sum_{r=0}^{k-1}(\bbS^r\bbE\bbS^{k-r}+\bbS^{r+1}\bbE\bbS^{k-r-1})] (\bbv_{Tt}\otimes\bbv_i) \nonumber \\
	&=\bbS_T^l\bbv_{Tt} \otimes \sum_{r=0}^{k-1}(\bbS^r\bbE\bbS^{k-r}+\bbS^{r+1}\bbE\bbS^{k-r-1})\bbv_i.
	\label{mixedproduct}
\end{align}
With the eigenvalue definition $\bbS\bbv_i = \lambda_i\bbv_i$, we can reduce (\ref{mixedproduct}) into
\begin{equation}
	\lambda_{T,t}^l\bbv_{T,t} \otimes \sum_{r=0}^{k-1}(\lambda_i^{k-r}\bbS^r+\lambda_i^{k-r-1}\bbS^{r+1})\bbE\bbv_i.
	\label{evreplaced}
\end{equation}

By applying Lemma~\ref{mainlemma} on~(\ref{evreplaced}), we have
\begin{equation}
	\lambda_{Tt}^l\bbv_{Tt} \otimes\sum_{r=0}^{k-1}2m_i\lambda_i^k\bbv_i +(\lambda_i^{k-r}\bbS^r+\lambda_i^{k-r-1}\bbS^{r+1})\bbE_U\bbv_i
	\label{lemmareplaced}
\end{equation}
where recall $m_i$ is the $i$-th eigenvector of $\bbM$ and $\bbE_U = \bbE - \bbV\bbM\bbV^\herm$.
Then, by replacing (\ref{lemmareplaced}) in (\ref{bigone}) we get
\begin{align}
	&\| \hat{\bby} - \bby \|_2= \left\|\sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}\sum_{k=0}^{\bar{K}}\sum_{l=0}^{\tilde{K}} h_{kl} \label{newbigone} \right.\\
	&\left.\lambda_{Tt}^l\bbv_{Tt} \otimes\sum_{r=0}^{k-1}2m_i\lambda_i^k\bbv_i +(\lambda_i^{k-r}\bbS^r+\lambda_i^{k-r-1}\bbS^{r+1})\bbE_U\bbv_i\right\|_2. \nonumber
\end{align}
The first term of inner summation in~\eqref{newbigone}
\begin{equation}
	\bbt_1 = 2\sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}m_i\sum_{k=0}^{\bar{K}}\sum_{l=0}^{\tilde{K}} k h_{kl}\lambda_{Tt}^l\lambda_i^k (\bbv_{Tt}\otimes\bbv_i)
\end{equation}
can be simplified based on partial derivation definition
\begin{equation}
	\bbt_1 = 2\sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}m_i \lambda_i\frac{\partial h(\lambda_{Tt},\lambda_i)}{\partial \lambda_i} (\bbv_{Tt}\otimes\bbv_i).
	\end{equation}
Using inequalities~\eqref{eq:lipsch} and $\|\bbE\|\leq \eps$, we can bound the norm of this term by
\begin{equation}
	\|\bbt_1\|_2 \leq 2C\eps\|\bbx_\diamond\|_2 
	\label{1sttermbound}
\end{equation}
where $C$ is the integral Lipschitz constant of graph-time convolutional filters. 

For the second term of the inner summation in~\eqref{newbigone}, we use the mixed-product property again to write
\begin{align}
	\bbt_2 = \sum_{t=1}^{T}\sum_{i=1}^{N}\tilde{\bbx}_{ti}&(\bbI_T\otimes \bbV) 
	(\bbI_T \otimes \diag(\bbg_i)) \label{secondterm} \\
	&(\bbI_T\otimes \bbV^H)(\bbI_T\otimes \bbE_U) (\bbv_{Tt}\otimes\bbv_i), \nonumber
	\end{align}
where 
\begin{align}
	[\bbg_i]_j &= \sum_{k=0}^{\bar{K}}\sum_{l=0}^{\tilde{K}} k h_{kl}\lambda_{Tt}^l\sum_{r=0}^{k-1}\lambda_i^{k-r}\lambda_j^r+\lambda_i^{k-r-1}\lambda_j^{r+1} \label{gdef} \\
	&=\left\{
	\begin{matrix*}[l]
		&\lambda_i\frac{\partial h(\lambda_{Tt},\lambda_i)}{\partial \lambda_i} & \text{if}\quad i=j \\
		&\frac{\lambda_i+\lambda_j}{\lambda_i-\lambda_j}(h(\lambda_{Tt},\lambda_i)-h(\lambda_{Tt},\lambda_j))&\text{if}\quad i=j
		\end{matrix*}
	\right.. \nonumber
	\end{align}
From the integral Lipschitz filter (Def.~\ref{def:intlip}), each entry of $\bbg_i$ is bounded by $2C$, hence the operator norm of $\|\diag(\bbg_i)\|\leq 2C$.
Due to the Lemma~1 $\|\bbE_U\|\leq \eps\delta$, and then $\| \bbI_T \otimes \bbE_U \|$ is bounded by $\eps\delta\sqrt{T}$.
Finally, the summation over all frequency components multiplies the bound by $\sqrt{NT}$, so
\begin{equation}
	\|\bbt_2\|_2 \leq 2C\eps\delta T \sqrt{N} \|\bbx_{\diamond}\|_2.
	\label{2ndtermbound}
\end{equation}

Replacing~\eqref{1sttermbound} and~\eqref{2ndtermbound} bounds into~\eqref{newbigone} followed by triangle inequality leads to the upper bound on the filter output
\begin{equation}
	\|\hat{\bby} - \bby\|_2 \leq 2C\eps(1+\delta T \sqrt{N}) \|\bbx_\diamond\|_2 = \Delta \eps \|\bbx_\diamond\|_2
	\label{eq:filterbound}
\end{equation}
where $\Delta = 2C(1+\delta T \sqrt{N})$.

\smallskip
\noindent\textbf{GTCNN.}
We can write the output difference of a GTCNN with $L$ layers over the nominal graph $\bbx_{\diamond,L}$ and perturbed graph $\hat{\bbx}_{\diamond,L}$ as
\begin{align}
	&\|\bbx_{\diamond,L} - \hat{\bbx}_{\diamond,L}  \|_2 \leq \label{gtcnn_output_diff} \\
	&\left\|
	\sigma\left(\sum_{g=1}^F \bbH_L^{fg}\bbx_{\diamond,L-1}^g\right) - 
	\sigma\left(\sum_{g=1}^F \hat{\bbH}_L^{fg}\hat{\bbx}_{\diamond,L-1}^g\right)
	\right\|_2,
	\nonumber
\end{align}
where, for the sake of notation simplicity, $\bbH_L^{fg}$ and $\hat{\bbH}_L^{fg}$ are standing for $\bbH_L^{fg}(\bbS_T,\bbS)$ and $\bbH_L^{fg}(\bbS_T,\hat{\bbS})$, respectively.

Applying the 1-Lipschitz continuous property of activation function $|\sigma(a)-\sigma(b)|\leq |a-b|$, followed by triangular inequality leads into 
\begin{equation}
	\|\bbx_{\diamond,L} - \hat{\bbx}_{\diamond,L}  \|_2 \leq
	\sum_{g=1}^F \|\bbH_L^{fg}\bbx_{\diamond,L-1}^g - \hat{\bbH}_L^{fg}\hat{\bbx}_{\diamond,L-1}^g \|_2.
	\label{gtcnn_output_diff_simple}
\end{equation}
Adding and subtracting $\hat{\bbH}_L^{fg}\bbx_{\diamond,L-1}^g$ and leveraging again the triangular inequality we can upper bound~\eqref{gtcnn_output_diff_simple} as 
\begin{align}
	\|\bbx_{\diamond,L} - \hat{\bbx}_{\diamond,L}  \|_2 &\leq 
	\|(\bbH_L^{fg}-\hat{\bbH}_L^{fg})\bbx_{\diamond,L-1}^g\|_2 \nonumber\\
	&+\|\hat{\bbH}_L^{fg}(\bbx_{\diamond,L}^g-\hat{\bbx}_{\diamond,L-1}^g)\|_2.
	\label{gtcnn_addsub}
\end{align}
The first term is bounded by $\Delta\eps$ [cf.~\eqref{eq:filterbound}] being it related to the filter stability.
The second term is bounded by spectral response of graph-time convolutional filters $\|\hat{\bbH}_L^{fg}\|\leq 1$ based on the theorem assumption [cf. Def~\ref{def:norm}].
Replacing these bounds into~\eqref{gtcnn_addsub} leads to
\begin{equation}
	\|\bbx_{\diamond,L} - \hat{\bbx}_{\diamond,L}  \|_2 \leq
	\sum_{g=1}^F \Delta \eps \|\bbx_{\diamond,L-1}^g\|_2 +  \|\bbx_{\diamond,L-1}^g-\hat{\bbx}_{\diamond,L-1}^g\|_2.
	\label{gtcnn_bound_raw}
\end{equation}
This equation indicates a recursion where the bound in the last layer depends on the bound in the previous layer.
We can write the output norm of each layer as
\begin{equation}
	\|\bbx_{\diamond,\ell}^f\|_2 \leq \sum_{g=1}^F \|\bbx_{\diamond,\ell-1}^g \|_2
	\label{gtcnn_bound_layers}
\end{equation}
Substituting~\eqref{gtcnn_bound_raw} and~\eqref{gtcnn_bound_layers} and solving the recursion bounds as in~[(87)-(88), 13] we can bound the output difference norm as
\begin{equation}
	\|\Phi(\bbx_{\diamond};\bbS_T,\bbS)-\Phi(\bbx_{\diamond};\bbS_T,\hat{\bbS})\|_2 \leq
	L F^{L-1}\Delta\eps \|\bbx_\diamond\|_2.
\end{equation}

